SUNAR: Semantic Uncertainty based Neighborhood Aware Retrieval for Complex QA

Complex question-answering (QA) systems face significant challenges in retrieving and reasoning over information that addresses multi-faceted queries. While large language models (LLMs) have advanced the reasoning capabilities of these systems, the bounded-recall problem persists, where procuring all relevant documents in first-stage retrieval remains a challenge. Missing pertinent documents at this stage leads to performance degradation that cannot be remedied in later stages, especially given the limited context windows of LLMs which necessitate high recall at smaller retrieval depths. In this paper, we introduce SUNAR, a novel approach that leverages LLMs to guide a Neighborhood Aware Retrieval process. SUNAR iteratively explores a neighborhood graph of documents, dynamically promoting or penalizing documents based on uncertainty estimates from interim LLM-generated answer candidates. We validate our approach through extensive experiments on two complex QA datasets. Our results show that SUNAR significantly outperforms existing retrieve-and-reason baselines, achieving up to a 31.84% improvement in performance over existing state-of-the-art methods for complex QA.

==> 03-framework.tex <==
\section{Methodology}
\label{sec:methods}

% In this section, we describe our approach \name{} which employs LLM-guided Neighborhood Aware Retrieval (NAR) to improve the quality of documents with a limited budget for LLM-based complex QA. An overview of the proposed approach \name{} is shown in Figure \ref{fig:main} and Algorithm \ref{alg: main}. \name{} comprises an \textit{Neighborhood Aware Retrieval} component (Section \ref{sec:adaptive_retrieval}) which is guided by an \textit{Answer Semantic Uncertainty (ASU)} (Section \ref{sec:answer_uncertainty} component. This is coupled with a \textit{Meta Evidence Reasoning} (MER) component that helps refine the step-by-step reasoning path from the query understanding component and the re-ranked evidence from ASU component aggregated across all sub-questions. 

The common approach to performing open-domain QA tasks typically involves a two-step process: retrieval of relevant information followed by a reasoning or QA step using the retrieved contexts. While this method works well for simpler questions, complex questions often consist of multiple sub-questions, necessitating more involved query understanding techniques, such as decomposing the main question into its constituent parts before retrieval. 
For complex questions, after decomposition, the retrieval step is followed by a ranking process, often performed by a fine-tuned model, to ensure that the most relevant documents are selected for reasoning. This ranking is crucial, especially due to the limited input capacity of large language models (LLMs), which restricts the amount of context they can process at once. 
Finally, the reasoning step is applied, where the LLM processes the selected, ranked contexts to generate the final answer. In this work, we adopt an LLM as the core question-answering model to handle the reasoning and answer generation phases.


\input{algo-SUNAR}
\subsection{Complex Question Answering}

Given a set of complex questions with corresponding answers $D = \{(q_1,a_1),...,(q_n,a_n)\}$, where $n$ is the total size, $q_i \in Q$ (set of questions), $a \in A$ (set of answers); the question decomposition models usually attempt to generate a decomposition.
We define a decomposition for a question-answer(QA) pair $(q,a)$ as
$de(q,a) = \{(sq_1,R_1,sa_1),..., (sq_k,R_k,sa_k)\}$, $k=k_{(q,a)}$ is the number of sub-questions for a given question $(q,a)$ and $(sq_i,sa_i)$ are the pairs of sub-question and corresponding answers, $R_i$ is a list of top-$l$ ranked documents (where $l$<=10) $[d_1..d_l]$ for a sub-question $sq_i$. We discuss the retrieval mechanism employed in Section \ref{sec:adaptive_retrieval}. The set $de = de(q,a)$ can be seen as a rationale, which is an ordered set for reasoning to arrive at a correct answer $a \in A$. In the reasoning chain, each sub-question $sq_j$ follows the answer to the previous question $sq_i$. The final answer $a$ can be seen as an aggregation of all the answers $sa_i,...,sa_k$ to the sub-questions \cite{dua-etal-2022-successive,decomposing_complex_multi_hop}.
\subsection{Neighborhood Aware Retrieval}
\label{sec:adaptive_retrieval}
Traditional RAG pipelines usually employ an off-the-shelf first-stage retriever for fetching relevant knowledge. While query understanding /question decomposition can help fetch better documents, the performance of complex QA is still limited by the quality of the first-stage retriever. To overcome the recall limitations of first-stage retrieval, we adopt Neighborhood Aware Retrieval (NAR) which employs the \textit{clustering hypothesis}~\cite{jardine1971use} which suggests that documents in the vicinity of highly scored documents tend to answer the same queries/questions. NAR first constructs a document-neighborhood graph $G = (V, E)$, also called the neighborhood graph. Each document is a node and the top-$k$ nearest neighbors are the edges, documents which are in the close vicinity (hence, $|E|=k|V|$) according to semantic relatedness. The neighborhood graph is constructed using a dense retriever if sparse retrieval is used for first-stage retrieval and vice versa to capture complementary signals. The neighborhood graph construction is a one-time activity for each document collection, and during inference, the indexed graph is directly used for lookup for efficiency. NAR starts with an initial set of ranked documents $R_0$ obtained from first-stage retrieval. NAR scores the documents in batches, each of size $b$, in each iteration till budget $c$ is reached (stopping condition in Line 15 of Algorithm \ref{alg: main}. NAR comprises a dynamically updated ranking pool $C$ (initialized to $R_0$, line 2) and a dynamically adapted Frontier ($F$, initially empty, line 3). Firstly, NAR employs a cross-encoder based re-ranker to score top $b$ documents from $P$ which constitute a batch $B$ (line 5). After this step, in LLM guided NAR (lines 6-8) we employ LLM-based feedback to re-score the documents in batch $B$. While we further elaborate on this in Section \ref{sec:answer_uncertainty}, vanilla NAR does not include this re-scoring step and adds $B$ to $R^+$ (line 9). Then the documents of the batch $B$ are removed from $F$ and $R_0$ as they are already ranked. Following this step, the neighbors of documents in $B$ are looked up from the neighborhood graph $G$. These documents, barring those already ranked are added to the frontier (line 13) prioritized according to the ranking score of the source document in $B$. NAR then explores a batch of documents from frontier $F$ instead of the next batch from $R_0$. This ensures the final ranked list includes documents not only from $R_0$ but additional documents also that are not included in the initial retrieval $R_0$. This aids in overcoming the recall limitations of first-stage retrieval. NAR proceeds by alternating between $R_0$ and $F$ till budget $c$ is reached and the final ranked list $R^+$ is returned. Note that NAR is invoked for each sub-question $sq_i$.
\subsection{LLM feedback for Neighborhood Aware Retrieval}
\label{sec:answer_uncertainty}
To improve the re-ranking of documents and promote the most relevant documents in the limited top-$l$ budget (for instance, where $l$=10), 
we propose an LLM-based feedback mechanism to re-score the top-ranked documents from the cross-encoder for each batch of NAR. While the cross-encoder aids in re-rank the retrieved documents for each sub-question from a relevance perspective, the LLM feedback helps re-score documents from an uncertainty perspective.

More formally, given the sub-question and ranked list of documents $R$ from the batch in the current iteration of NAR  $(sq_1, B)$, where $B=[d_1,d_2,...,d_b]$, the ASU (Answer Semantic Uncertainty) re-scores the documents and returns the batch $B$ with updated scores (Lines 6-8 of Algorithm \ref{alg: main}).
\begin{equation}
B = \mathtt{LLM\_SCORE}(sq_1,B)
\label{eq:rescore}
\end{equation}

It accomplishes this by first estimating answer consistency based on the number of answer semantic sets. This is computed by first estimating multiple answers for a given sub-question and ranked document list
\begin{equation}
   \{sa_1..sa_m\} = \phi(\bP_{LLM}(sq_1,R),m)
   \label{eq:response_gen}
\end{equation}
where $\phi$ is the response generator that generates multiple responses ($sa_1...sa_{m}$) from the distribution $\bP_{LLM}$. We further define $\sigma$ as the estimator of answer semantic sets through semantic equivalence estimation for semantic clustering. A semantic set is defined as a set of sequences that share the same meaning following the work \cite{kuhn2023semantic}. $\sigma$ takes as input a set of answers and outputs the number of answer semantic sets. 

\begin{equation}
\{ac_1..ac_s\} = \sigma(\{(sa_1,sa_2)..(sa_{m-1},sa_m)\})
\label{eq:sigma}
\end{equation}
where s denotes the number of semantic sets

It accomplishes this by clustering equivalent answers to the same answer semantic set through bi-directional entailment computed between each pair of answers. We employ bi-directional entailment as it is a stronger criterion for semantic equivalence \cite{kuhn2023semantic}. For instance,
\begin{equation}
\sigma(sa_i,sa_j) = M_{NLI}(sa_i | sa_j) \& M_{NLI}(sa_j | sa_i)
\label{eq:nli}
\end{equation}

 The above condition is checked for each pair, and two answer sequences are assigned to the same sequence only if they entail each other. If not, the answer sequences are assigned to distinct semantic sets. We posit that more semantic sets indicate that the LLM is uncertain about the answer to the given question and the current batch of documents. Finally, we re-score the documents in the current batch by penalizing the scores from the cross-encoder as follows 
 \begin{equation}
      \mathtt{LLM\_SCORE}(sq_1,B) = [\frac{sc_1}{s}.. \frac{sc_n}{s}]
      \label{eq:re-score-2}
 \end{equation}

 where, $sc_i$ refers to the cross-encoder score for ith document for a given sub-question in batch $B$. The above process is repeated for all batches till the budget $c$ for NAR is reached for a given sub-question. This is followed by the answer generation step using the LLM by leveraging top-10 documents from the re-ranked list. The same is repeated for all sub-questions till the decomposition stops and the final answer is generated.

 However, we observe that in this sequential reasoning process, the final answer is derived solely based on answers to previous sub-questions and only the evidence for the last sub-question. Hence, any errors in intermediate steps could result in cascading errors resulting in wrong final answer. Inspired by post-hoc LLM correction strategies, we propose a simple yet significantly effective Meta Evidence Reasoner (MER) to tackle this issue. The MER component leverages the reasoning path obtained through sequential reasoning $[(sq_1,sa_1...(sq_n,sa_n)]$ and the top-k evidences from the set of ranked list of documents ${R_1^+, R_2^+...}$ across sub-questions and prompts the LLM with the original question to obtain the final answer. The prompt is as shown in Figure \ref{fig:repair_prompt}.  

==> algo-sunar-v2.tex <==
\begin{algorithm}[H]
  \SetAlgoLined
\caption{The \name{} Algorithm} 
\label{alg: main}
\begin{algorithmic}[1]
\Require Initial retrieved list $R$, batch size $b$, re-ranking budget $c$, document graph $G$
\Ensure Re-Ranked pool $R^+$

  // Initialize re-ranking results
  \State $R^+ \gets \emptyset$

  // Initialize re-ranking pool
  \State $C \gets R$

  // Initialize neighbor pool
  \State $N \gets \emptyset$

\doWhile{$|R^+| < c$}

    // Ranker: Select top $b$ documents, subject to budget $c$
    \State $B \gets$ \Call{Score}{top $b$ from $P$, subject to $c$}

    // Generate multiple responses using language model
    \State $\{sa_1...sa_m\} \gets \phi(\bP_{LLM}(sq_1,B))$

    // Apply semantic clustering on the responses
    \State $\{ac_1..ac_s\} \gets \sigma(sa_1..sa_m)$

    // Rescore batch using number of semantic sets
    \State $B \gets$ \Call{rescore}{$B$, $1/s$}

    // Add batch to re-ranked results
    \State $R^+ \gets R^+ \cup B$

    // Remove batch from initial ranking
    \State $R \gets R \setminus B$

    // Remove batch from neighbor pool
    \State $N \gets N \setminus B$

    // Update frontier by adding neighbors of batch, excluding already re-ranked
    \State $N \gets N \cup (\Call{Neighbours}{B, G} \setminus R^+)$

    // Alternate between re-ranking pool and neighbor pool
    \State $C \gets \begin{cases} 
        R & \text{if}\; C = F \\
        N & \text{if}\; C = N \\
    \end{cases}$

\endDoWhile

\end{algorithmic}
\end{algorithm}

==> auto-cot-prompt.tex <==
\begin{table}[htb!!]
\begin{tcolorbox}[title=Prompt: Auto Chain of Thought]
\small
\textbf{\ding{228} \textsc{System Message}}: You are tasked with providing rationale and answers to timeline-based queries about various subjects. \newline
Your reply should try to be as complete as possible. Think of the subject's past and contributions. Try to think step by step. Write down your thinking process. \newline
After you provide an answer, you will next be tasked to extract the timelines from there, which should answer the first question best. 

The timeline should be structured like this: \vspace{0.2cm}

Each answer should be structured as a list, with different entries for each subject or title. Each entry must include the years corresponding to the following the title or subject. \vspace{0.2cm}

Please adhere to the following structure in your responses: \\
- Write the title or name first, exactly as it would appear in a formal context such as Wikipedia. \\
- Follow the title or name with a colon and then the years. \\
- Represent a range of years by using a short dash. \\
- Separate multiple years or ranges with a comma and a space. \\
- End each entry with a comma, except for the last entry. \\
- If the current year is relevant to the query, use "2024" instead of "present". \\
- Each answer should be on a new line, with no additional characters or explanations. \\
- Ensure the completeness and correctness of your answers. Try to be as complete as possible. \\
- If provided examples, follow the examples structure and reasoning style. \vspace{0.2cm}

\textbf{Example response format:} \\
\texttt{Title or Name: year1-year2, year3} \\
\texttt{Title or Name: Years}, \vspace{0.2cm}

\textbf{\ding{228} \textsc{User Message (Example)}}: \textit{List all political positions Greg Abbott held to this day.} \\

% Indicate automatic rationale generation below
\textbf{\ding{228} \textsc{Assistant Message (Auto-Generated Rationale)}}: 
 \textit{Greg Abbott is a prominent American politician and officeholder. He first served as Justice of the Supreme Court in Texas from 1996 to 2001. In 2002, Abbott was elected as the 50th Attorney General of Texas. In 2014, he announced his candidacy for Governor of Texas, winning the election and taking office in 2015. Abbott has continued to serve as Governor to this day. Additionally, between 2019 and 2020, Abbott was the Chair of the Republican Governors Association.} \newline  

\textbf{\ding{228} \textsc{User Message}}: \textit{Extract the timeline, including both years and answers from your previous answer now. }\\ \\ 
\textbf{\ding{228} \textsc{Assistant Message (Example)}}:
\textit{"Governor of Texas": 2015-2024,} \newline
\textit{"Chair of the Republican Governors Association": 2019-2020,} \newline
\textit{"50th Attorney General of Texas": 2002-2015,} \newline
\textit{"Justice of the Supreme Court of Texas": 1996-2001} \\ 

\textbf{\ding{228} \textsc{User Message}}: \textit{List all political positions Brian Pallister held to this day.} 
\end{tcolorbox}
\captionof{figure}{Auto COT prompt setup (closed book setting)}
\label{fig:timeline_rationale_prompt}
\end{table}


==> error_analysis.tex <==

\begin{table*}[h!]
    \centering
    \begin{tabular}{p{7.4cm} p{7.4cm}}
    \toprule
        %     \multicolumn{2}{l}{ {\color{olive}\textit{CONTENT WARNING: potentially objectionable content}} } \\
        % \midrule
    \multicolumn{2}{l}{\ding{228} \textbf{Query}: \texttt{List all teams  Alan Kirby played to this day.}} \\
    \midrule
    \textbf{Expected Answer} & \textbf{\textbf{Generated Answer} } \\
    \midrule

    \vspace{-10pt} % Manually adjust vertical space
    \begin{itemize}[leftmargin=*,topsep=0pt,partopsep=0pt,parsep=0pt,itemsep=0pt]
        \item Aston Villa F.C.: 1996-1998, 1994-1996
        \item Johnville F.C. (Waterford): 1994
        \item Republic of Ireland under-21 national football team: 1998
        \item Waterford United F.C.: 1999-2001
        \item League of Ireland XI: 2010
        \item Longford Town F.C.: 2001-2006, 2012
        \item St Patrick's Athletic F.C.: 2007-2008
        \item Sporting Fingal F.C.: 2009-2010
        \item Sligo Rovers F.C.: 2011
    \end{itemize}
    
    
    
            & I apologize, but I couldn't find any information on a person named Alan Kirby playing for any football teams. If you meant someone else or provided incorrect information, please let me know and I'll be happy to help.  \\
    
    \bottomrule
    \end{tabular}
    \caption{Example of query that the model is not able to answer. Generated with Meta Llama 3 with manual 3-shot prompting. }
    \label{tab:refusal_example}
    
\end{table*}

\begin{table*}[h!]
    \centering
    \begin{tabular}{p{7.4cm} p{7.4cm}}
    \toprule
    \multicolumn{2}{l}{\ding{228} \textbf{Query}: \texttt{List all teams Alan Kirby played to this day.}} \\
    \midrule
    \textbf{Expected Answer} & \textbf{Generated Answer} \\
    \midrule
    \vspace{-10pt}
    \begin{itemize}[leftmargin=*,topsep=0pt,partopsep=0pt,parsep=0pt,itemsep=0pt]
        \item Aston Villa F.C.: 1996-1998, 1994-1996
        \item Johnville F.C. (Waterford): 1994
        \item Republic of Ireland under-21 national football team: 1998
        \item Waterford United F.C.: 1999-2001
        \item League of Ireland XI: 2010
        \item Longford Town F.C.: 2001-2006, 2012
        \item St Patrick's Athletic F.C.: 2007-2008
        \item Sporting Fingal F.C.: 2009-2010
        \item Sligo Rovers F.C.: 2011
    \end{itemize}
    
    &
    \vspace{-10pt}
    \begin{itemize}[leftmargin=*,topsep=0pt,partopsep=0pt,parsep=0pt,itemsep=0pt]
    \item Leeds United F.C.: 1995-2001, 2000 
    \item England national under-21 football team: 1999 
    \item Huddersfield Town A.F.C.: 2001-2004
    \item Rotherham United F.C.: 2004-2006 
    \item Doncaster Rovers F.C.: 2006-2008 
    \item Grimsby Town F.C.: 2008-2010 
    \item Bradford City A.F.C.: 2010-2011 
    \item Gainsborough Trinity F.C.: 2011-2012 
    \item Harrogate Railway Athletic F.C.: 2012-2013 
    \item Farsley Celtic F.C.: 2013-2014 
    \item York City F.C.: 2014-2015
    \item Brighouse Town A.F.C.: 2015-2016 
    \item AFC Emley F.C.: 2016-2017
    \item Garforth Town A.F.C.: 2017-2018 
    \item Liversedge F.C.: 2018
    \end{itemize}
    
    \\
    \bottomrule
    \end{tabular}
    \caption{Example of model answer with incorrect details. }
    \label{tab:hallucination_model_answer}
\end{table*}
\begin{table*}[h!]
    \centering
    \begin{tabular}{p{7.4cm} p{7.4cm}}
    \toprule
    \multicolumn{2}{l}{\ding{228} \textbf{Query}: \texttt{List all political positions Ulf Kristersson held to this day.}} \\
    \midrule
    \textbf{Expected Answer} & \textbf{Generated Answer} \\
    \midrule
    \vspace{-10pt}
    \begin{itemize}[leftmargin=*,topsep=0pt,partopsep=0pt,parsep=0pt,itemsep=0pt]
        \item Prime Minister of Sweden: 2022-2024
        \item \textcolor{red}{Leader of the Moderate Party: 2017-2024}
        \item Leader of the Opposition: 2017-2022
        \item Minister for Social Security: 2010-2014
        \item Chairman of the Moderate Youth League: 1988-1992
        \item \textcolor{red}{Member of the Riksdag: 2014-2024, 1991-2000}
    \end{itemize}
    
    &
    \vspace{-10pt}
    \begin{itemize}[leftmargin=*,topsep=0pt,partopsep=0pt,parsep=0pt,itemsep=0pt]
    \item \textcolor{red}{Leader of the Moderate Party: 2017-2024}
    \item \textcolor{red}{Member of the Riksdag: 2006-2021, 2022-2024}
    \end{itemize}
    
    \\
    \bottomrule
    \end{tabular}
    \caption{Example of incomplete answer}
    \label{tab:incomplete_answer}
\end{table*}


==> exemplars-qualitative.tex <==



\begin{table*}
\begin{tabular}{lp{.98\textwidth}}
\toprule
    \textbf{Method} & \textbf{Exemplars} \\
\midrule
\small

LENS  & \textbf{Question}: A cat chases a rat 6 hours after the rat runs. cat takes 4 hours to reach the rat. If the average speed of the cat is 90 kmph, what s the average speed of the rat?
\\ & \textbf{Options}: ['A)32kmph', 'B)26kmph', 'C)35kmph', 'D)36kmph', 'E)32kmph']
\\ & \textbf{Rationale:} Cat take 10 hours and rat take 4 hours...then Distance is 90*4.so speed of rat is (90*4)/10 = 36kmph 
\textbf{Answer: D}
 \\\cline{2-2}
 & \textbf{Question:}  A business executive and his client are charging their dinner tab on the executive's expense account.The \dots?
 \\ & \textbf{Options}: ['A)69.55\$', 'B)50.63\$', 'C)60.95\$', 'D)52.15\$', 'E)53.15'] \\
 & \textbf{Rationale}:  let x is the cost of the food
1.07x is the gross bill after including sales tax
1.15* 1.07x=75 \textbf{Answer}: C \\\cline{2-2}
 & \textbf{Question:}John and David were each given X dollars in advance for each day they were expected to perform at a community festival. John eventually,\dots? 
 \\ &\textbf{Options}: 'A)11Y', 'B)15Y', 'C)13Y', 'D)10Y', 'E)5Y' \textbf{Rationale:} \dots  \textbf{Answer:} A\\\cline{2-2}
  & \textbf{Question:}A contractor undertakes to do a piece of work in 40 days. He engages 100 men at the beginning and 100 more after 35 days and completes the work in stipulated time. If he had not engaged the additional men, how many days behind schedule would it be finished?? \\
 & \textbf{Options}: 'A)2', 'B)5', 'C)6', 'D)8', 'E)9'
  \textbf{Rationale:}  [(100$\times$ 35)+(200$\times$ 5)] men can finish the work in 1 day
therefore 4500 men can finish the work in 1 day. 100 men can finish it in  $\frac{4500}{100}$ = 45 days.
This is 5 days behind Schedule 
  \textbf{Answer:} A\\\cline{2-2}
    & \textbf{Question:} A can do a job in 9 days and B can do it in 27 days. A and B working together will finish twice the amount of work in ------- days? \\
 & \textbf{Options}: 'A)22 days', 'B)18 days', 'C)22 6/2 days', 'D)27 days', 'E)9 days'
  \textbf{Rationale:} 1/9 + 1/27= 3/27 = 1/9
9/1 = 9*2 =18 day
  \textbf{Answer:} B\\
  \midrule

  
\colorg \static{} & \colorg \textbf{Question}: The average age of three boys is 15 years and their ages are in proportion 3:5:7. What is the age in years of the youngest boy?
\\ \colorg & \colorg \textbf{Options}: ['A)9', 'B)10', 'C)11', 'D)12', 'E)13']
\\\colorg & \colorg\textbf{Rationale:}3x + 5x + 7x = 45,
x =3,
3x = 9
\textbf{Answer: A}
 \\\cline{2-2}\colorg
 & \colorg\textbf{Question:}  Can you deduce the pattern and find the next number in the series? $6, 14, 26, 98$?

  \textbf{Options}: [''A)276', 'B)277', 'C)278', 'D)279', 'E)None of these']] \\\colorg
 & \colorg\textbf{Rationale}:  $6 = 1^1 + 2^1 + 3^1, 
14 = 1^2 + 2^2 + 3^2,
36 = 1^3 + 2^3 + 3^3,
98 = 1^4 + 2^4 + 3^4$
Thus the next number 
 \textbf{Answer}: A \\\cline{2-2}\colorg
 & \colorg\textbf{Question:}In covering a distance of 42 km, A takes 2 hours more than B. If A doubles his speed, then he would take 1 hour less than B. A's speed is:? 
\\ \colorg & \colorg \textbf{Options}: 'A)5 km/h', 'B)7 km/h', 'C)10 km/h', 'D)15 km/h', 'E)25 km/h' \textbf{Rationale:} Let A's speed be X km/hr.
Then, 42/x - 42/2x = 3
6x = 42
x = 7 km/hr \textbf{Answer:} B\\\cline{2-2}\colorg
  &\colorg \textbf{Question:}Find  the number which when multiplied by 15 is increased by 196. \\\colorg
 &\colorg \textbf{Options}: 'A)14', 'B)20', 'C)26', 'D)28', 'E)30'
  \textbf{Rationale:}  Solution
Let the number be x .
Then, 15x - x = 196
‹=›14x = 196
x ‹=› 14 
  \textbf{Answer:} A\\\cline{2-2}\colorg
    & \colorg\textbf{Question:} A certain sum of money at simple interest amounted Rs.980 in 3 years at 5\% per annum, find the sum? \\\colorg
 & \colorg\textbf{Options}: 'A)867', 'B)855', 'C)299', 'D)852', 'E)903'
  \textbf{Rationale:} 980 = P [1 + (3*5)/100]
P = 852 
  \textbf{Answer:} D\\
\midrule
\midrule
\end{tabular}
\caption{Qualitative analysis of exemplars for \textbf{\aqua{}} dataset selected by LENS vs \static{}. Rationale is not completely shown for some questions to conserve space. However, in our experiments all exemplars include rationales.}
\label{tab:exemplar_qualitative_aquarat}
%\vspace{-0.25cm}
\end{table*}





















\begin{table*}
\begin{tabular}{lp{.98\textwidth}}
\toprule
    \textbf{Method} & \textbf{Exemplars} \\
\midrule
\small

LENS  & \textbf{Table}: | increase ( decrease ) |
average yield | 2.75\% ( 2.75 \% ) |
volume | 0.0 to 0.25 |
energy services | 2013 |
fuel recovery fees | 0.25 |
recycling processing and commodity sales | 0.25 to 0.5 |
acquisitions / divestitures net | 1.0 |
total change | 4.25 to 4.75\% ( 4.75 \% ) |
\\ & \textbf{Question}: what is the ratio of the acquisitions / divestitures net to the fuel recovery fees as part of the expected 2019 revenue to increase
\\ & \textbf{Rationale:} ans=( 1.0 / 0.25 )
\textbf{Answer: }  The answer is 4
 \\\cline{2-2}
 & \textbf{Table:}  ( in millions ) | 2009 | 2008 | 2007 |
sales and transfers of oil and gas produced net of production andadministrative costs |  -4876 ( 4876 ) |  -6863 ( 6863 ) |  -4613 ( 4613 ) |
\dots
 \\ & \textbf{Question}: were total revisions of estimates greater than accretion of discounts?
\\
 & \textbf{Rationale}: \dots   \textbf{Answer}: The answer is yes  \\\cline{2-2}
 & \textbf{Table:} | 2007 | 2008 | change |
capital gain distributions received | 22.1 |  5.6 | -16.5 ( 16.5 ) |
other than temporary impairments recognized | -.3 ( .3 ) | -91.3 ( 91.3 ) | -91.0 ( 91.0 ) |
net gains ( losses ) realized onfund dispositions | 5.5 | -4.5 ( 4.5 ) | -10.0 ( 10.0 ) |
net gain ( loss ) \dots
 \\ &\textbf{Question}: what percentage of tangible book value is made up of cash and cash equivalents and mutual fund investment holdings at december 31 , 2009?
\textbf{Rationale:} ( 1.4 / 2.2 )  \textbf{Answer:}  The answer is 64\%\\\cline{2-2}
  & \textbf{Table:} in millions | 2009 | 2008 | 2007 |
sales | 5680 | 6810 | 6530 |
operating profit | 1091 | 474 | 839 |
\\
 & \textbf{Question}: north american printing papers net sales where what percent of total printing paper sales in 2009?
   \textbf{Rationale:} x0=( 2.8 * 1000 ), ans=( x0 * 5680 )
  \textbf{Answer:} The answer is 49\%\\\cline{2-2}
    & \textbf{Table:}  in millions | december 312015 | december 312014 |
total consumer lending | 1917 | 2041 |
total commercial lending | 434 | 542 |
total tdrs | 2351 | 2583 |
nonperforming | 1119 | 1370 |
\dots
 \\
 & \textbf{Question}: what was the change in specific reserves in alll between december 31 , 2015 and december 31 , 2014 in billions?
  \textbf{Rationale:} ( .3 - .4 )
  \textbf{Answer:}  The answer is -0.1\\
  \midrule

  
\colorg \static{} & \colorg \textbf{Table}: | 2008 | 2007 |
balance at beginning of year | 23.2 | 56.4 |
additions due to acquisition of allied | 582.9 | 2014 |
additions based on tax positions related to current year | 10.6 | 16.3 |
reductions for tax positions related to the current year | -5.1 ( 5.1 ) | -17.2 ( 17.2 ) |
\dots
\\ \colorg & \colorg \textbf{Question}: in 2008 what was the change in the gross unrecognized tax benefits in millions
\\\colorg & \colorg\textbf{Rationale:}  (611.9 - 23.2 )
\textbf{Answer: } The answer is 588.7
 \\\cline{2-2}\colorg
 & \colorg\textbf{Table:} december 31 2004 | 1054 |
december 31 2005 | 1216 |
december 31 2006 | 1219 |
december 31 2007 | 2566 |
  \textbf{Question}: what was devon's average translation adjustments included in accumulated other comprehensive income ( in millions ) from 2004 through 2007?
\textbf{Rationale}: x0=( 1054 + 1216 ), x1=( x0 + 1219 ), x2=( x1 + 2566 ), ans=( x2 + 4 )
 \textbf{Answer}: The answer is 1513.75 \\\cline{2-2}\colorg
 & \colorg\textbf{Table:} | 2016 | 2015 ( in thousands ) | 2014 |
share-based compensation expense | 30809 | 21056 | 29793 |
income tax benefit | 9879 | 6907 | 7126 |
\\ \colorg & \colorg \textbf{Question}:  how much percent did the income tax benefit increase from 2014 to 2016?
  \\\colorg  & \colorg  \textbf{Rationale:}  x0=( 9879 - 7126 ), ans=( x0 - 7126 )
 \textbf{Answer:} The answer is increased 38.6\%\\\cline{2-2}\colorg
  &\colorg \textbf{Table:}  in billions | 2018 |
january 1 |  33.3 |
issuances | 4.5 |
calls and maturities | -6.8 ( 6.8 ) |
other | -.1 ( .1 ) |
december 31 | 30.9 |
\\\colorg
 &\colorg \textbf{Question}: assuming all matured securities were pledged as collateral , how much should we assume came from the calls?
  \textbf{Rationale:}  ans=( 6.8 - 4.9 ) 
  \textbf{Answer:} The answer is 1.9 \\\cline{2-2}\colorg
    & \colorg\textbf{Table:}  in millions of dollars | u.s . | outside u.s . | december 31 2008 | december 31 2007 |
commercial and similar letters of credit | 2187 | 6028 | 8215 | 9175 |
 \dots\\\colorg
 & \colorg\textbf{Question}: what percentage of citigroup 2019s total other commitments as of december 31 , 2008 are outside the u.s.?
  \textbf{Rationale:}  ans=( 236931 / 1349500 )
  \textbf{Answer:} The answer is 18\%\\
\midrule
\midrule
\end{tabular}
\caption{Qualitative analysis of exemplars for \textbf{\fin{}} dataset selected by LENS vs \static{}. Rationale is not completely shown for some questions to conserve space. However, in our experiments all exemplars include rationales.}
\label{tab:exemplar_qualitative_fin}
%\vspace{-0.25cm}
\end{table*}
















\begin{table*}
\begin{tabular}{lp{.98\textwidth}}
\toprule
    \textbf{Method} & \textbf{Exemplars} \\
\midrule
\small

LENS  & \textbf{Question}: Michael wants to dig a hole 400 feet less deep than twice the depth of the hole that his father dug. The father dug a hole at a rate of 4 feet per hour. If the father took 400 hours to dig his hole \dots ?
\\ & \textbf{Rationale:} Since the father dug a hole with a rate of 4 feet per hour, if the father took 400 hours digging the hole, he dug a hole 4*400 = 1600 feet deep. \dots Michael will have to work for 2800/4 = 700 hours.
\textbf{Answer:} 700
 \\\cline{2-2}
 & \textbf{Question:} When Erick went to the market to sell his fruits, he realized that the price of lemons had risen by $4$ for each lemon. The price of grapes had also increased by half the price that \dots?
 \\ & \textbf{Rationale}:  The new price for each lemon after increasing by $4$ is $8+4 =12$ For the 80 lemons, \dots Erick collected $140*9=1260$ From the sale of all of his fruits, Erick received $1260+960 =2220$.
 \\ & \textbf{Answer}: 2220 \\\cline{2-2}
 & \textbf{Question:}James decides to build a tin house by collecting 500 tins in a week. On the first day, he collects 50 tins. On the second day, he manages to collect 3 times that number. \dots? 
 \\ &\textbf{Rationale:} On the second day, he collected 3 times the number of tins he collected on the first day, which is $3*50 =150$ tins. \dots he'll need to collect $200/4=50$ tins per day to reach his goal. \\&\textbf{Answer:} 50\\\cline{2-2}
  & \textbf{Question:} Darrel is an experienced tracker. He can tell a lot about an animal by the footprints it leaves behind. Based on the impressions, he could tell the animal was traveling east at 15 miles per hour \dots ? \\
 & \textbf{Rationale:} If we let x be the amount of time, in hours, it will take for Darrel to catch up to the coyote, \dots If we subtract 1 x from each side, we get x=1, the amount of time in hours.
 \textbf{Answer:} 1\\\cline{2-2}
    & \textbf{Question:} Martha needs to paint all four walls in her 12 foot by 16 foot kitchen, which has 10 foot high ceilings \dots If Martha can paint 40 square feet per hour, how many hours will it take her to paint kitchen? 
  \\&\textbf{Rationale:} There are two walls that are 12' by 10' and two walls that are 16' by 10' \dots how many hours she needs to finish: 1680 sq ft / 40 sq ft/hour = 42 hours 
  \textbf{Answer:} 42\\
  \midrule

  
\colorg \static{} & \colorg \textbf{Question}: The difference between the number of boys and girls in a tree planting event is 400. If there are 600 boys at the event, and the number of girls is more than the number of boys \dots ?
\\ \colorg & \colorg \textbf{Rationale:}  If there are 600 boys at the event, and the difference between boys and girls is 400, there are 600+400=1000 girls.
\dots 60\% of the total number of boys and girls at the event is 60/100*1600=960
\textbf{Answer:} 960
 \\\cline{2-2}\colorg
 & \colorg\textbf{Question:}  Casey is trying to decide which employee she wants to hire. One employee works for $\$20$ an hour. The other employee works for $\$22$ an hour, but Casey would also get a $\$6$/hour subsidy \dots ?
\\\colorg  & \colorg\textbf{Rationale}:  First find the weekly cost of the first employee: \$20/hour * 40 hours/week = 800/week \dots subtract the smaller weekly cost from the bigger weekly cost: \$800/week - \$640/week = 160/week.
 \textbf{Answer}: 160 \\\cline{2-2}\colorg
 & \colorg\textbf{Question:}Cara has 60 marbles in a bag. 20 of them are yellow, half as many are green, \dots If Cara picks a marble at random, what are the odds it's blue (expressed as a percentage)?
\\ \colorg & \colorg \textbf{Rationale:} First find the number of green marbles: 20 yellow marbles/2=10 green marbles. \dots find the percentage chance of getting a blue marble: 15 marbles/60 marbles*100=25\%.
\textbf{Answer:} 25\\\cline{2-2}\colorg
&\colorg \textbf{Question:} Samir just turned half the age Hania was 10 years ago. If in five years Hania will be 45 years old, what will Samir's age be five years from now?
 \\\colorg  &\colorg 
\textbf{Rationale:} If in five years, Hania will be 45 years old, currently she is 45-5=40 years old. Ten years ago, Hania was 40-10=30 years old. \dots In five years, Samir will be 15+5=20 years old. 
\textbf{Answer:} 20\\\cline{2-2}\colorg
& \colorg\textbf{Question:} If the normal hours of operation of Jean's business are 4 pm to 10p every day Monday through Friday, and from 6 pm to 10 pm on weekends, how many hours is the business open in a week?
\\\colorg
& \colorg \textbf{Rationale:} First, we find the number of hours per weekday by subtracting the smaller number from the larger one \dots We add these two totals together to find that 30+8=38 hours per week.
\textbf{Answer:} 38\\
\midrule
\midrule
\end{tabular}
\caption{Qualitative analysis of exemplars for \textbf{\gsm{}} dataset selected by LENS vs \static{}. Rationale is not completely shown for some questions to conserve space. However, in our experiments all exemplars include rationales.}
\label{tab:exemplar_qualitative_gsm8k}
%\vspace{-0.25cm}
\end{table*}











\begin{table*}
\begin{tabular}{lp{.98\textwidth}}
\toprule
    \textbf{Method} & \textbf{Exemplars} \\
\midrule
\small

LENS  & \textbf{Table}: | Name | Age (years)
| Jessica | 2
| Dalton | 7
| Kelsey | 5
| Lamar | 8
| Alexis | 2
 \textbf{Question}: A girl compared the ages of her cousins. What is the median of the numbers?
\textbf{Rationale:} Read the numbers from the table: 2, 7, 5, 8, 2.
First, arrange the numbers from least to greatest: 2, 2, 5, 7, 8.
Now find the number in the middle. The number in the middle is 5.
The median is 5.
\textbf{Answer: } 5
 \\\cline{2-2}
 & \textbf{Table:} | City | Number of houses sold 
| Melville | 878
| New Hamburg | 871
| Charles Falls | 881
| Pennytown | 817
\textbf{Question}: A real estate agent looked into how many houses were sold in different cities. Where were the fewest houses sold? \textbf{Rationale}: Find the least number in the table. \dots The least number is 817.
Now find the corresponding city. Pennytown corresponds to 817.
   \textbf{Answer}: 817  \\\cline{2-2}
 & \textbf{Table:} | Day | Number of new customers
| Saturday | 2
| Sunday | 2
| Monday | 9
| Tuesday | 4
| Wednesday | 10
| Thursday | 3
| Friday | 6
\textbf{Question}: A cable company analyst paid attention to how many new customers it had each day. What is the median of the numbers?
\textbf{Rationale:} Read the numbers \dots Now find the number in the middle. The number in the middle is 4.
The median is 4.
  \textbf{Answer:} 4 \\\cline{2-2}
  & \textbf{Table:} | Day | Number of cups
| Friday | 8
| Saturday | 4
| Sunday | 10
| Monday | 6
| Tuesday | 6
| Wednesday | 1
| Thursday | 0
 \textbf{Question}: Nancy wrote down how many cups of lemonade she sold in the past 7 days. What is the range of the numbers?
\textbf{Rationale:} Read the numbers from the table: 8, 4, 10, 6, 6, 1, 0. \dots Subtract the least number from the greatest number: 10-0=10. The range is 10.
\textbf{Answer:} 10\\\cline{2-2}
    & \textbf{Table:}  | Price | Quantity demanded | Quantity supplied
|\$700 | 9,800 | 22,600
|\$740 | 8,000 | 22,800
|\$780 | 6,200 | 23,000
|\$820 | 4,400 | 23,200
|\$860 | 2,600 | 23,400
\textbf{Question}: At a price of \$860, is there a shortage or a surplus?
 \textbf{Rationale:} At price of \$860, quantity demanded is less than quantity supplied. There is too much of the good or service for sale at that price. So, there is a surplus.
 \textbf{Answer:}  surplus\\
 \midrule

  
\colorg \static{} & \colorg \textbf{Table}: | Day | Number of tickets
| Monday | 36
| Tuesday | 43
| Wednesday | 46
| Thursday | 59
| Friday | 37
| Saturday | 46
| Sunday | 51
\textbf{Question}: The transportation company tracked the number of tickets sold in the past 7 days. What is the range of the numbers?
\textbf{Rationale:} Read the numbers from the table: 36, 43, 46, 59, 37, 46, 51. Find greatest number. The greatest number is 59. Find least
number. The least number is 36. Subtract least from the greatest number: 59 - 36 = 23.
The range is 23.
\textbf{Answer: } 23
 \\\cline{2-2}\colorg
 & \colorg\textbf{Table:} | Stem | Leaf 
| 4 | 2, 7, 9, 9, 9
| 5 | 1
| 6 | 9
| 7 | 2, 2, 3, 3, 5
| 8 | 
| 9 | 0
\textbf{Question}:  A pottery factory kept track of the number of broken plates per shipment last week. How many shipments had exactly 73 broken plates?
\textbf{Rationale}:  For the number 73, the stem is 7, and the leaf is 3. Find the row where the stem is 7. In that row, count all the leaves equal to 3.
You counted 2 leaves, which are blue in the stem-and-leaf plot above. 2 shipments had exactly 73 broken plates.
\textbf{Answer}: 2 \\\cline{2-2}\colorg
 & \colorg\textbf{Table:} | purple and red clay bead | \$0.02
| small pink bead | \$0.04
| pearl bead | \$0.07
| round silver bead | \$0.01
| brown cat's eye bead | \$0.08
| orange glass bead | \$0.07
\textbf{Question}:  Kylie has \$0.05. Does she have enough to buy a small pink bead and a purple and red clay bead?
\textbf{Rationale:}  Add the price of a small pink bead and the price of a purple and red clay bead: \$0.04 + \$0.02 = \$0.06
\$0.06 is more than \$0.05. Kylie does not have enough money.
\textbf{Answer:} Kylie does not have enough money.  \\\cline{2-2}\colorg
  &\colorg \textbf{Table:}  | Price | Quantity demanded | Quantity supplied
| \$165 | 17,900 | 6,400
| \$345 | 15,100 | 8,900
| \$525 | 12,300 | 11,400
| \$705 | 9,500 | 13,900
| \$885 | 6,700 | 16,400
\textbf{Question}: Look at the table. Then answer the question. At a price of \$885, is there a shortage or a surplus?
\textbf{Rationale:}  At the price of \$885, the quantity demanded is less than the quantity supplied. There is too much of the good or service for sale at that price. So, there is a surplus.
\textbf{Answer:} surplus \\\cline{2-2}\colorg
& \colorg\textbf{Table:} | Chickenville | 3:00 A.M. | 12:00 P.M. | 3:30 P.M.
| Floral Gardens | 3:45 A.M. | 12:45 P.M. | 4:15 P.M.
| Pleasant River Campground | 4:45 A.M. | 1:45 P.M. | 5:15 P.M.
| Happy Cow Farm | 5:15 A.M. | 2:15 P.M. | 5:45 P.M.
| Rocky Ravine Town | 5:45 A.M. | 2:45 P.M. | 6:15 P.M.
\textbf{Question}: Look at the following schedule. Doug just missed the 3.00 A.M. train at Chickenville. How long does he have to wait until the next train?
\textbf{Rationale:}  Find 3:00 A. M. in the row for Chickenville. Look for the next train in that row.
The next train is at 12:00 P. M. The elapsed time is 9 hours.
\textbf{Answer:} 9\\
\midrule
\midrule
\end{tabular}
\caption{Qualitative analysis of exemplars for \textbf{\tab{}} dataset selected by LENS vs \static{}. Rationale is not completely shown for some questions to conserve space. However, in our experiments all exemplars include rationales.}
\label{tab:exemplar_qualitative_tabmwp}
%\vspace{-0.25cm}
\end{table*}



















\begin{table*}
\begin{tabular}{lp{.98\textwidth}}
\toprule
    \textbf{Method} & \textbf{Exemplars} \\
\midrule
\small

LENS & \textbf{Facts}: Penguins are native to the deep, very cold parts of the southern hemisphere. Miami is located in the northern hemisphere and has a very warm climate.
 \\&\textbf{Question:} Would it be common to find a penguin in Miami?
\\ & \textbf{Rationale:} Where is a typical penguin's natural habitat? What conditions make \#1 suitable for penguins? Are all of \#2 present in Miami?
\textbf{Answer: No}
 \\\cline{2-2}
 & \textbf{Facts:} Shirley Bassey recorded the song Diamonds are Forever in 1971. Over time, diamonds degrade and turn into graphite. Graphite is the same chemical composition found in pencils.
\\ &\textbf{Question:} Is the title of Shirley Bassey's 1971 diamond song a true statement?
 \textbf{Rationale}: What is the title to Shirley Bassey's 1971 diamond song? Do diamonds last for the period in \#1? \textbf{Answer}: No \\\cline{2-2}
 & \textbf{Facts:} The first six numbers in the Fibonacci sequence are 1,1,2,3,5,8. Since 1 is doubled, there are only five different single digit numbers.  \textbf{Question:} Are there five different single-digit Fibonacci numbers?
 \\ &\textbf{Rationale:} What are the single-digit numbers in the Fibonacci sequence? How many unique numbers are in \#1? Does \#2 equal 5?
\textbf{Answer:} Yes\\\cline{2-2}
  & \textbf{Facts:} Katy Perry's gospel album sold about 200 copies. Katy Perry's most recent pop albums sold over 800,000 copies.
\textbf{Question:} Do most fans follow Katy Perry for gospel music?
 \textbf{Rationale:} What type of music is Katy Perry known for? Is Gospel music the same as \#1?
 \textbf{Answer:} No\\\cline{2-2}
    & \textbf{Facts:} The Italian Renaissance was a period of history from the 13th century to 1600. A theocracy is a type of rule in which religious leaders have power. Friar Girolamo Savonarola was the ruler of Florence, after driving out the Medici family, from November 1494 â€ 23 May 1498. \textbf{Question:} Was Florence a Theocracy during Italian Renaissance?
  \textbf{Rationale:} When was the Italian Renaissance?When did Friar Girolamo Savonarola rule Florence? Is \#2 within the span of \#1? Did Friar Girolamo Savonarola belong to a religious order during \#3?
  \textbf{Answer:} Yes\\
  \midrule




  
\colorg \static{} & \colorg \textbf{Facts}: The average cost of a US Boeing 737 plane is 1.6 million dollars. Wonder Woman (2017 film) grossed over 800 million dollars at the box office. \textbf{Question}: Is a Boeing 737 cost covered by Wonder Woman (2017 film) box office receipts?
 \textbf{Rationale:}  How much does a Boeing 737 cost?. How much did the 2017 movie Wonder Woman gross? Is \#2 greater than \#1?
\textbf{Answer:} Yes
 \\\cline{2-2}\colorg
 & \colorg \textbf{Facts}: Big Show is a professional wrestler that weighs 383 pounds. Force is equal to mass times acceleration. An adult Cheetah weighs around 160 pounds. An adult Cheetah can run up to 58 MPH. \textbf{Question:}  Can a cheetah generate enough force to topple Big Show?
\colorg\textbf{Rationale}:  How much does Big Show weigh? How much does a cheetah weigh? How fast can a cheetah run? Is the force produced by a mass of \#2 and a speed of \#3 enough to knock over something that weighs \#1?
 \textbf{Answer}: Yes \\\cline{2-2}\colorg
 & \colorg \textbf{Facts}: Spaghetti and meatballs are a staple on Italian pizzeria menus in the US. The Olive Garden, an Italian family restaurant, has several dishes with meatballs. Meatballs originated in the Chinese Qin dynasty (221 BC to 207 BC). \textbf{Question:} Do restaurants associate meatballs with the wrong country of origin?
 \textbf{Rationale:} In what country is the oldest evidence of people eating meatballs found? What dish involving meatballs became popular in the United States after being invented in New York City in the 20th century? With which national cuisine do Americans typically associate \#2? Are \#3 and \#1 different?
\textbf{Answer:} Yes\\\cline{2-2}\colorg
&\colorg \textbf{Facts:} Torah scrolls must be duplicated precisely by a trained scribe. The Torah has a total of 8,674 words. The population of Bunkie Louisiana is 3,939 people according to a 2018 census. \\ \colorg &\colorg \textbf{Question:} Can you give at least one word from the Torah to all residents of Bunkie Louisiana?
\textbf{Rationale:} How many words are in the Torah? How many residents does Bunkie, Louisiana have? Is \#1 greater than \#2?
\textbf{Answer:} Yes\\\cline{2-2}\colorg
&\colorg \textbf{Facts:} Wrestlemania X took place in 1994. The Toyota Prius was first manufactured in 1997. \textbf{Question:} Could someone have arrived at Wrestlemania X in a Toyota Prius?
\textbf{Rationale:} When did Wrestlemania X hold? When was the Toyota Prius first manufactured? Is \#2 before \#1?
\textbf{Answer:} No\\
\midrule
\midrule
\end{tabular}
\caption{Qualitative analysis of exemplars for \textbf{\strat{}} dataset selected by LENS vs \static{}. Rationale is not completely shown for some questions to conserve space. However, in our experiments all exemplars include rationales.}
\label{tab:exemplar_qualitative_strategyqa}
%\vspace{-0.25cm}
\end{table*}

==> figures/ablation/sunar_comp_mqa.tex <==

\begin{tikzpicture}
\edef\mylst{"44.58","45.75","54.83"}
\edef\explora{"24.84","0","28.11","32.75","44.28"}

    \begin{axis}[
            ybar=5pt,
            width=4.2cm,
            height=5cm,
            bar width=0.25,
            every axis plot/.append style={fill},
            grid=major,
            xtick={1, 2, 3},
            xticklabels={ PRF, self-ask,\textbf{\name{}}},
            xlabel={},
            ylabel style = {font=\tiny},
        yticklabel style = {font=\boldmath \tiny,xshift=0.05ex},
        xticklabel style ={font=\tiny,yshift=0.5ex},
            ylabel={Task Performance (cover-EM)},
            enlarge x limits=0.25,
            ymin=0,
            ymax=80,
            nodes near coords style={font=\tiny,align=center,text width=2em},
            legend cell align={left},
            legend pos=north west,
            legend columns=-1,
    extra y tick style={grid=major,major grid style={thick,draw=black}}, 
            legend style={/tikz/every even column/.append style={column sep=0.5cm}},
        ]
        \addplot+[
            ybar,
            plotColor1*,
            nodes near coords=\pgfmathsetmacro{\mystring}{{\mylst}[\coordindex]}\textbf{\mystring},
            nodes near coords align={vertical},
            draw=black,
            postaction={
                    pattern=north east lines
                },
        ] plot coordinates {
                (1,44.58)
                (2,45.75)
                (3,54.83)
            };
            
        \draw[color=black, style=densely dashed,line width = 1.5pt] (axis cs:0,65.55) -- (axis cs:5,65.55)  node[pos=0.2, anchor=west, font=\small, yshift=7pt] {Gold};           
    %     \addplot+[
    %         ybar,
    %         plotColor2*,
    %         draw=black,
    %         nodes near coords=\pgfmathsetmacro{\mystring}{{\explora}[\coordindex]}\textbf{\mystring},
    % nodes near coords align={vertical},
    %         postaction={
    %                 pattern=north west lines
    %             },
    %     ] plot coordinates {
    %             (1,24.84)
    %             (2,0)
    %             (3,28.11)
    %             (4,32.75)
    %             (5,44.28 )
    %         };
 

    \end{axis}


    
\end{tikzpicture}


==> figures/answer_distribution_plot.tex <==
\begin{figure}[ht]
    \begin{tikzpicture}
        \begin{axis}[
            ybar,
            ymin=0, ymax=14,
            xtick=data,
            ylabel={Average Number of Answers},
            symbolic x coords={\textbf{Ground Truth}, Manual Mistral, KNN Mistral, Manual COT Mistral, Auto COT Mistral, Manual Llama, KNN Llama, Manual COT Llama, Auto Llama},
            x tick label style={rotate=70, anchor=east, font=\scriptsize},
            ylabel style={font=\small},
            width=0.7\textwidth,
            height=0.4\textwidth,
            bar width=8pt,
            grid=major,
            error bars/.cd,
            y dir=both, y explicit,
            legend style={font=\small},
            % nodes near coords,
            % nodes near coords align={vertical},
            every node near coord/.append style={font=\footnotesize}
        ]

        % Plot all bars with default styles
        \addplot+[
            ybar,
            error bars/.cd,
            y dir=both, y explicit
        ] plot coordinates {
            (Ground Truth, 8.64) +- (0, 4.83)
            (Manual Mistral, 3.90) +- (0, 2.91)
            (KNN Mistral, 4.57) +- (0, 2.90)
            (Manual COT Mistral, 4.01) +- (0, 2.18)
            (Auto COT Mistral, 4.58) +- (0, 2.60)
            (Manual Llama, 4.71) +- (0, 2.56)
            (KNN Llama, 5.73) +- (0, 3.06)
            (Manual COT Llama, 4.16) +- (0, 1.99)
            (Auto COT Llama, 3.23) +- (0, 2.39)
        };

        \legend{Average ± Std. Dev.}
        \end{axis}
    \end{tikzpicture}
    \caption{Average number of answers with standard deviations for the different prompting strategies for Mistral and Meta LLama}
    \label{fig:avg_answers}
\end{figure}

==> figures/top_k_mqa.tex <==


\begin{tikzpicture}
\edef\mylst{"24.12","25.80","49.58","52.5","54.83"}

    \begin{axis}[
            ybar=5pt,
            width=4.6cm,
            height=5cm,
            bar width=0.25,
            every axis plot/.append style={fill},
            grid=major,
            xtick={1, 2, 3, 4 , 5},
            xticklabels={ 1, 3, 5,7,10},
            xlabel={},
            ylabel style = {font=\tiny},
        yticklabel style = {font=\boldmath \tiny,xshift=0.05ex},
        xticklabel style ={font=\tiny,yshift=0.5ex},
            ylabel={Task Performance (cover-EM)},
            enlarge x limits=0.25,
            ymin=0,
            ymax=75,
            nodes near coords style={font=\tiny,align=center,text width=2em},
            legend cell align={left},
            legend pos=north west,
            legend columns=-1,
    extra y tick style={grid=major,major grid style={thick,draw=black}}, 
            legend style={/tikz/every even column/.append style={column sep=0.5cm}},
        ]
        \addplot+[
            ybar,
            plotColor1*,
            draw=black,
            nodes near coords=\pgfmathsetmacro{\mystring}{{\mylst}[\coordindex]}\textbf{\mystring},
    nodes near coords align={vertical},
            postaction={
                    pattern=north west lines
                },
        ] plot coordinates {
                (1,46.91)
                (2,48.58)
                (3,49.58)
                (4,52.5)
                (5,54.83)


            };
            
               

 

    \end{axis}


    
\end{tikzpicture}


==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

% \color{purple}
% Is our method specific to in-context numerical reasoning, or can it also work for other NLU tasks? What is special about numerical reasoning? Can we say that we design a general method but test it on numerical reasoning tasks because they are more difficult? \color{green} As semantic similarity between train and test set can't be used to select ICEs in case of numerical reasoning. Therefore we propose EXPLORA.\\
% \color{black}
% \color{blue}
% - We are given only the task-specific loss, which is different from generative model error. We do not utilize the logits given by generative models. Bayesian explanation, in-context one iteration GD -- each of these papers, can we say why these theories don't apply to complex QA.

% Complex numerical reasoning tasks such as financial question answering \cite{chen2022finqa} or tabular question answering \cite{tabmwp} require both language understanding as well as reasoning skills.
% Large language models (LLMs) have been shown to exhibit both these skills.
% Language understanding skills help  While 

% \color{gray}

Answering complex questions that require multi-step numerical reasoning \cite{chen2022finqa,tabmwp,aqua_rat,roy2016solving} over structured and unstructured sources is an active research area with applications in finance, law, and healthcare~\cite{wang2023survey}.
% The complexity in such tasks could arise from multiple factors, such as the need to parse heterogeneous sources like tables and text \cite{chen2022finqa} coupled with multi-step numerical reasoning \cite{tabmwp,aqua_rat,roy2016solving} to answer the question. 

Existing supervised approaches for numerical reasoning involve fine-tuning of multiple generative models for generating arithmetic programs or stepwise solution to the original problem \cite{chiang-chen-2019-semantically,amini-etal-2019-mathqa,aqua_rat,roy2016solving,geva-etal-2020-injecting,cobbe2021training}. 
 
% However, existing approaches require expensive annotations of supervised stepwise rationales along with the solution for fine-tuning multiple generative models \cite{aqua_rat} \cite{cobbe2021training} \cite{geva-etal-2020-injecting} lacking a general purpose solution. 

\begin{figure*}[t]
\centering

\includegraphics[width=0.8\textwidth]{figures/explora-cropped.pdf}\\
\caption{Overview of \static{}, proposed exemplar selection approach.}
\label{fig:icl}
% \vspace{-4mm}
\end{figure*}


More recently, the advances in Large Language Models (LLMs) has lead to substantial progress in a wide range of natural language understanding and reasoning tasks \cite{brown2020gpt3}. The emergent capabilities in LLMs\cite{wei2022emergent,gpt3incontext} such as In-Context Learning (ICL) has paved the way to a new class of approaches that employ chain-of-thought reasoning~\cite{complex_cot} \cite{wei2023chainofthought} for solving complex numerical reasoning questions.
Instead of fine-tuning task-specific models, these approaches focus on choosing carefully constructed exemplars with rationales to be used as input to LLMs, commonly termed as prompting.
% A distinct advantage of prompting with demonstration samples vs fine-tuning is  that the LLM is a general-purpose machine that can be used to solve multiple numerical reasoning tasks.
% In this paper, our focus is to propose a general framework that can be employed to solve multiple QA tasks that require numerical reasoning over homogeneous and heterogeneous sources by selecting suitable demonstration samples.

\mpara{The limitations of manual exemplar selection.} 
% It is inherently hard for the LLMs to perform multi-step reasoning using few-shot in-context learning with just the  \texttt{(input, output)} pairs~\cite{rae2022scaling}.
To tackle complex numerical reasoning problems, \textit{chain-of-thought} (COT) prompting was proposed to add hand-crafted natural language rationales (stepwise solutions) to the prompts in addition to input and output resulting in \texttt{(input, rationale, output)}~\cite{wei2023chainofthought}.
% The process of generating stepwise natural language rationales can be seen as decomposing the original problem to simpler problems that can be solved with less effort \cite{wei2023chainofthought} \cite{brown2020gpt3}.

% Interesting, 
% COT rationales for compositional natural language questions involve generating explanations for the final answer. 
% However, such explanations have been found to be unfaithful to the reasoning process of underlying LLM \cite{turpin2023language,ye2022unreliability} for answering compositional questions in complex QA, unlike numerical reasoning questions. 
% In such cases, the decomposition of such question to simpler sub-questions is observed to be more faithful. To induce such decomposition capabilities in LLMs, authors of the work self-ask \cite{self_ask} modify COT prompting and propose to add hand-crafted follow-up questions derived from the original complex questions to the prompt.
However, there are inherent limitations of COT approach for complex and hybrid numerical reasoning tasks. 
The COT involves the manual effort of selecting the best exemplars with appropriate rationales that sufficiently convey the  execution strategy for the task under consideration. The manual selection process is tedious and not scalable across different numerical reasoning tasks. Since the outputs generated by the LLM are highly sensitive to exemplars provided \cite{lu-etal-2022-fantastically,zhao2021calibrate,chang2023data}, it is crucial to select meaningful exemplars that are robust across evaluation samples and improve overall task performance.

\mpara{Limitations of automated exemplar selection approaches}:
To tackle these limitations, several automated exemplar selection approaches have been proposed \cite{ye2023compositional,lu-etal-2022-fantastically,rubin-etal-2022-learning,complex_cot}. These approaches are usually dynamic exemplar selection methods, which select several demonstration examples from the training set for each test example. Several approaches also require annotated data and training of several models for exemplar selection\cite{lu2023dynamic,ye2023compositional}. These approaches entail to heavy computational requirements during inference, especially when there is a large pool of exemplars to select from. While unsupervised approaches like similarity \cite{rubin-etal-2022-learning} or diversity based \cite{ye-etal-2023-complementary} approaches exist for dynamic exemplar selection, they also require projecting the input query and the entire pool of exemplars to a continuous vector space followed by search, increasing computational time during inference. Additionally, the majority of these approaches assume the exemplars chosen to be independent of each other and only consider the interaction between the test sample and the exemplars. They do not account for the interactions between the exemplars themselves.

 As an alternative to dynamic exemplar selection approaches, LENS \cite{li2023finding} proposed to select a static set of task level support exemplars. However, LENS assumes access to language model output logits and involves multiple expensive evaluations of the LLM for scoring the exemplars. LENS also does not model the interactions between exemplars and scores each sample independently. 
% In the example below, using Few-shot-COT results in inaccurate results due to lack of decomposition information in its prompt (hidden due to space reasons).
% \input{intro-example-mouth}

\mpara{\static{} (Static Exemplar Selection Approach):}
In this work, we propose a novel static exemplar selection method \static{}, that selects multiple high value/low loss exemplar subsets. An overview of the working of \static{} is shown in Figure \ref{fig:icl}. The selection of task level exemplar subsets are performed once, and we model the interactions between exemplars through initial sampling of subsets and by directly scoring and selecting subsets. We propose a parameterized scoring function that approximates the loss indicative of task performance using features from a transformer based embedding model. We propose an exploration mechanism as shown in Figure \ref{fig:icl} to estimate the parameters of the scoring function with minimal calls to the LLM and without access to logits from the LLM. Our approach mitigates the expensive processing during inference incurred by traditional dynamic exemplar selection approaches and obviates the need for manual exemplar selection while providing high performance.


\mpara{Contributions.} The core contributions of our work are:
\begin{description}
    \item 
    1) We propose a new robust static exemplar selection approach \static{}, that selects task level exemplars for numerical reasoning based questions.

    \item 
    2) We demonstrate the ability of transferring selected exemplars across models. We show that exemplars selected using smaller models can be used to induce reasoning capabilities in much larger models leading to reduced costs.
     \item 
     3) We demonstrate that \static{} is less resource intensive compared to existing approaches, as it results in minimal calls to the LLMs for exemplar selection.
    \item 
    4) We conduct extensive experiments with different exemplar selection methods to showcase the generalized performance of \static{} across multiple complex and hybrid numerical reasoning based QA tasks.
\end{description}

\color{black}


==> llama3.1_results.tex <==
\begin{table*}[ht]
\centering

\renewcommand{\arraystretch}{1.3} % Increase row height
\begin{tabular}{lccccc}
\toprule
\textbf{Model}  & \textbf{Precision} & \textbf{Recall} & \textbf{F1} & \textbf{Temporal Overlap} & \textbf{Time Jaccard} \\
\midrule
\rowcolor[gray]{0.93} \multicolumn{6}{l}{\textbf{Closed Book}} \\

\textbf{Meta Llama 3.1} & & & & & \\
\fshot{} & 0.48 & 0.376 & 0.397 & 0.466 & 0.398 \\ 
\knn{} \fshot{} & 0.464 & 0.415 & 0.414 & 0.495 & 0.421 \\
\COT{} & 0.511 & 0.399 & 0.412 & 0.578 & 0.446 \\ 
Auto COT{} & 0.381 & 0.302 & 0.31 & 0.439 & 0.356 \\ 

\rowcolor[gray]{0.93} \multicolumn{6}{l}{\textbf{Open Book}} \\
\textbf{BM25} & 0.606 & 0.530 & 0.540 & 0.658 & 0.603 \\
\textbf{all-minim-v2} & 0.444 & 0.389 & 0.393 & 0.479 & 0.425  \\
\textbf{multi-qa-mpnet} & 0.416 & 0.340 & 0.353 & 0.468 & 0.379 \\

\rowcolor[gray]{0.93} \multicolumn{6}{l}{\textbf{Golden Evidence}} \\
\textbf{Meta Llama 3.1} & & & & & \\
\fshot{} & 0.922 & 0.837 & 0.866 & 0.880 & 0.861 \\ 
\knn{} \fshot{} & 0.928 & 0.886 & 0.899 & 0.940 & 0.925 \\ 
\bottomrule
\end{tabular}
\caption{Performance of various models on the benchmark using different prompting techniques (Llama 3.1)}
\label{tab:llama_3_1}
\end{table*}


==> manual-cot-prompt.tex <==
\begin{table}[htb!!]
\begin{tcolorbox}[title=Prompt: Manual Chain of Thought]
\small
\textbf{\ding{228} \textsc{System Message}}: You are tasked with providing rationale and answers to timeline-based queries about various subjects. \newline
Your reply should be structured in this format: \texttt{Rationale: \{your rationale\} /n Final answer: \{your answer\}} \vspace{0.2cm}

Each answer should be structured as a list, with different entries for each subject or title. Each entry must include the years corresponding to the following the title or subject. \vspace{0.2cm}

Please adhere to the following structure in your responses: \\
- Write the title or name first, exactly as it would appear in a formal context such as Wikipedia. \\
- Follow the title or name with a colon and then the years. \\
- Represent a range of years by using a short dash. \\
- Separate multiple years or ranges with a comma and a space. \\
- End each entry with a comma, except for the last entry. \\
- If the current year is relevant to the query, use "2024" instead of "present". \\
- Each answer should be on a new line, with no additional characters or explanations. \\
- Ensure the completeness and correctness of your answers. Try to be as complete as possible. \\
- If provided examples, follow the example structure and reasoning style. \vspace{0.2cm}

\textbf{\ding{228} \textsc{User Message (Example)}}: \textit{List all political positions Greg Abbott held to this day.} \\ \vspace{0.2cm}

\textbf{\ding{228} \textsc{Assistant Message (Example)}}: \newline 
\texttt{Rationale}: \textit{Greg Abbott is an American politician and officeholder. He was first known to be the Justice of the Supreme Court in Texas. He started in 1996 and resigned in 2001. In 2002, he got elected as the 50th Attorney General of Texas. In 2014, Abbott announced his candidacy for Governor of Texas. He won the elections and became Governor of Texas in 2015. To this day, he still holds this office. Between 2019 and 2020, he was also the Chair of the Republican Governors Association.} \newline
\texttt{Final answer:} \newline
\textit{"Governor of Texas": 2015-2024,} \newline
\textit{"Chair of the Republican Governors Association": 2019-2020,} \newline
\textit{"50th Attorney General of Texas": 2002-2015,} \newline
\textit{"Justice of the Supreme Court of Texas": 1996-2001} \\ \vspace{0.2cm}

\textbf{\ding{228} \textsc{User Message}}: \textit{List all political positions Brian Pallister held to this day.} \vspace{0.2cm} \\ 

\end{tcolorbox}
\captionof{figure}{Manual COT prompt setup (closed book setting)}
\label{fig:rationale_prompt}
\end{table}


==> ndcg_plots.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/ndcg_plot.png}
    \caption{Comparison of retrieval models (nDCG) }
                \label{fig:retriever_extra_2}

\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/recall_plot.png}
    \caption{Comparison of retrieval models (Recall) }
                \label{fig:retriever_extra_1}

\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/precision_plot.png}
    \caption{Comparison of retrieval models (Precision). }
        \label{fig:retriever_extra}
\end{figure}

==> prompt-aqua.tex <==
\begin{table*}[hbt!]

\begin{tcolorbox}[title= AQUA Prompt]
\small
\textbf{Instruction}:\texttt{You are a helpful, respectful and honest assistant helping to solve math word problems or tasks requiring reasoning or math. Follow given examples and solve the problems in step by step manner.}



\paragraph{\textbf{Exemplars}}:

[Question]: \textit{ The average age of three boys is 45 years and their ages are in proportion 3:5:7. What is the age in years of the youngest boy?}

[Options]: A) 9, B) 10, C) 11, D) 12, E) 13

[Explanation]: \textsf{$3x + 5x + 7x = 45$, \\ $x =3$, \\ $3x = 9$}

[Answer]: \textcolor{teal}{\textsf{The option is A}}
\\
\dots \\
\dots 
\paragraph{\textbf{Test Input}}: Question: {}
Options: {}

Explanation: [INS]
Answer: [INS]

\end{tcolorbox}
\captionof{figure}{Prompt for \aqua{}}
\label{prompt:aqua} 
\end{table*}

==> prompt-finqa.tex <==
\begin{table*}[hbt!]

\begin{tcolorbox}[title= FinQA Prompt]
\small
\textbf{Instruction}:\texttt{You are a helpful, respectful and honest assistant helping to solve math word problems or tasks requiring reasoning or math, using the information from given table and text.}



\paragraph{\textbf{Exemplars}}:

% [Question]: \textit{what was the growth rate of reit index as of 12/31/2003}

% [Table]: ventas | $ 100 | $ 206 | $ 270 | $ 331 | $ 457 | $ 512 | 
% nyse composite index | $ 100 | $ 132 | $ 151 | $ 166 | $ 200 | $ 217 | 
% all reit index | $ 100 | $ 138 | $ 181 | $ 196 | $ 262 | $ 215 | 
% healthcare reit index | $ 100 | $ 154 | $ 186 | $ 189 | $ 273 | $ 279 | 
% russell 1000 index | $ 100 | $ 130 | $ 145 | $ 154 | $ 178 | $ 188 | 

% [Text]: \textit{stock performance graph the following performance graph compares the cumulative total return ( including dividends ) to the holders of our common stock from december 31 , 2002 through december 31 , 2007 , with the cumulative total returns of the nyse composite index , the ftse nareit composite reit index ( the 201call reit index 201d ) , the  \dots}

% [Program]: \textsf{ans=(( 138 - 100 )/100)*100}

% [Answer]: \textcolor{teal}{\textsf{38}}
% \\
% \dots \\
% \dots 
% \paragraph{\textbf{Test Input}}: Read the following table, and then answer the question:
% Table: {}
% Text: {}
% Question: {}

% Equation: [INS]
% Answer: [INS]





\textit{Read the following table, and then answer the question:}

[Table]: Year | 2016 | 2015 | 2014 |\\
share-based compensation expense | $30809$ | $21056$ | $29793$ | \\
income tax benefit | $9879$ | $6907$ | $7126$ |

[Question]: \textit{how much percent did the income tax benefit increase from 2014 to 2016?}

[Explanation]: \textsf{$x0=( 9879 - 7126$ ), \\ ans=( $x0 / 7126$ )}

[Answer]: \textcolor{teal}{\textsf{The answer is increased 38.6\%}}
\\
\dots \\
\dots 
\paragraph{\textbf{Test Input}}: Read the following table, and then answer the question:
Table: {}
Question: {}

Explanation: [INS]
Answer: [INS]




\end{tcolorbox}
\captionof{figure}{Prompt for \fin{}}
\label{prompt:finqa} 
\end{table*}

==> prompt-tabmwp.tex <==
\begin{table*}[hbt!]

\begin{tcolorbox}[title= TabMWP Prompt]
\small
\textbf{Instruction}:\texttt{You are a helpful, respectful and honest assistant helping to solve math word problems or tasks requiring reasoning or math, using the information from the given table. Solve the given problem step by step providing an explanation for your answer.}



\paragraph{\textbf{Exemplars}}:

[Table]: Table: Day | Number of tickets \\
Monday | $36$ \\
Tuesday | $43$ \\
Wednesday | $46$ \\
Thursday | $59$ \\
Friday | $37$ \\
Saturday | $46$ \\
Sunday | $51$ 


[Question]: \textit{The transportation company tracked the number of train tickets sold in the past 7 days. What is the range of the numbers?}

[Explanation]: \textsf{Read the numbers from the table. $36$, $43$, $46$, $59$, $37$, $46$, $51$ \\ First, find the greatest number. The greatest number is $59$. \\ Next, find the least number. The least number is $36$. \\ Subtract the least number from the greatest number: $59$ - $36$ = $23$}

[Answer]: \textcolor{teal}{\textsf{The range is 23}}
\\
\dots \\
\dots 
\paragraph{\textbf{Test Input}}: Table: {}
Question: {}

Explanation: [INS]
Answer: [INS]




\end{tcolorbox}
\captionof{figure}{Prompt for \tab{}}
\label{prompt:tabmwp} 
\end{table*}

==> prompt_gsm8k.tex <==
\begin{table*}[hbt!]

\begin{tcolorbox}[title= GSM8K Prompt]
\small
\textbf{Instruction}:\texttt{You are a helpful, respectful and honest assistant helping to solve math word problems or tasks requiring reasoning or math. Follow given examples and solve the problems in step by step manner.}



\paragraph{\textbf{Exemplars}}:

[Question]: \textit{Samir just turned half the age Hania was $10$ years ago. If in five years Hania will be $45$ years old, what will Samir's age be five years from now?}

[Explanation]: \textsf{If in five years, Hania will be $45$ years old, currently she is $45-5 = 40$ years old.\\
Samir just turned half the age Hania was $10$ years ago, which means she is $30/2 = 15$ years old. \\
In five years, Samir will be $15+5 = 20$ years old.}

[Answer]: \textcolor{teal}{\textsf{20 years old}}
\\
\dots \\
\dots 
\paragraph{\textbf{Test Input}}: Question: {}

Explanation: [INS]
Answer: [INS]

\end{tcolorbox}
\captionof{figure}{Prompt for \gsm{}}
\label{prompt:gsm8k} 
\end{table*}


==> prompt_strategy.tex <==
\begin{table*}[hbt!]

\begin{tcolorbox}[title= StrategyQA Prompt]
\small
\textbf{Instruction}:\texttt{You are a helpful, respectful and honest assistant helping to solve commonsense problems requiring reasoning. Follow the given examples that use the facts to answer a question by decomposing into sub-questions first and then predicting the final answer as "Yes" or "No" only.}



\paragraph{\textbf{Exemplars}}:

[Facts]: Snowden scored above $145$ on two separate IQ tests. The minimum accepted IQ score for MENSA on the Stanford–Binet is $132$, while for the Cattell it is $148$.

[Question]: \textit{Could Edward Snowden join MENSA?}

[Sub-question 1]: \textsf{What is the minimum accepted IQ score to be admitted to MENSA?\\}
[Sub-question 2]: \textsf{What is Edward Snowden's IQ?\\}
[Sub-question 3]: \textsf{Is \#2 greater than or equal to \#1?}


[Answer]: \textcolor{teal}{\textsf{Yes}}
\\
\dots \\
\dots 
\paragraph{\textbf{Test Input}}: Facts: {} Question: {}

Sub-question: [INS]
Answer: [INS]

\end{tcolorbox}
\captionof{figure}{Prompt for \strat{}}
\label{prompt:strategy} 
\end{table*}


==> qualitative_analysis.tex <==
\begin{table*}[t!]
\centering
 % \scalebox{0.8}{
% \begin{tabular}{p{2cm}p{1.3cm}p{1.3cm}p{1.3cm}}

\begin{tabular}{lccc}
\hline
\textbf{GAC}  ($\kappa$)& \textbf{GEU} ($\kappa_K$) & \textbf{AC} ($\kappa$) & \textbf{EU} ($\kappa$)\\ 
\hline

\midrule
 4.87$\pm$0.32 (0.77) & 4.93$\pm$0.24 (0.64)& 3.65$\pm$1.37 (0.86) & 3.35$\pm$1.68 (0.79) \\

% \numdecomp{}  & 0.779 & \textbf{0.581} \\
 
\bottomrule
\end{tabular}
% }
\caption{Manual evaluation. AC: Answer Completeness, EU : Evidence usefulness, G indicates Ground Truth. We use the Likert scale (1-5) and Cohen's Kappa ($\kappa$) for inter-annotator agreement (in brackets).}
\label{tab:question_quality}
\end{table*}



==> rag-prompt.tex <==
\begin{table}[htb!!]
\begin{tcolorbox}[title=Prompt: Retrieval Augmented Generation]
\small
\textbf{\ding{228} \textsc{System Message}}: You are tasked with responding to timeline-based queries about various subjects. \newline
Each response should be structured as a list, with different entries for each subject or title. Each entry must include the years corresponding to the title or subject. \newline
You will receive additional context from the user regarding the query. Use the context as additional sources to answer the query. \vspace{0.2cm}

Please adhere to the following structure in your responses: \\
- Write the title or name first, exactly as it would appear in a formal context such as Wikipedia. \\
- Follow the title or name with a colon and then the years. \\
- Represent a range of years by using a short dash. \\
- Separate multiple years or ranges with a comma and a space. \\
- End each entry with a comma, except for the last entry. \\
- If the current year is relevant to the query, use "2024" instead of "present". \\
- Each answer should be on a new line, with no additional characters or explanations. \\
- Ensure the completeness and correctness of your answers. \vspace{0.2cm}

\textbf{Example response format:} \\
\texttt{Title or Name: year1-year2, year3} \\
\texttt{Title or Name: Years}, \vspace{0.2cm}

% Show User Message and some context
\textbf{\ding{228} \textsc{User Message (Example)}}: \textit{List all political positions Joe Biden held to this day.} \vspace{0.2cm} \\
\textbf{Context:} \newline
\textit{Infobox: \newline
Order: 46th \newline
Office: President of the United States \newline
Vicepresident: Kamala Harris \newline
Term Start: January 20, 2021 \newline
Predecessor: Donald Trump \newline
... \newline
Other offices: \newline
Chair of the International Narcotics Control Caucus (2007–2009) \newline
Chair of the Senate Foreign Relations Committee (2001–2003, 2007–2009) \newline
Chair of the Senate Judiciary Committee (1987–1995) \newline
Member of the New Castle County Council (1971–1973)
} \\ \vspace{0.2cm}

% Assistant Message generated based on context
\textbf{\ding{228} \textsc{Assistant Message (Example)}}: \newline 
\textit{President of the United States (2021-2024)} \newline
\textit{Vice President of the United States (2009-2017)} \newline
\textit{United States Senator from Delaware (1973-2009)} \\ \vspace{0.2cm}

% New user message
\textbf{\ding{228} \textsc{User Message}}: \textit{List all political positions Brian Pallister held to this day.} \vspace{0.2cm} \\ 

\end{tcolorbox}
\captionof{figure}{RAG prompt (open book and golden evidence)}
\label{fig:timeline_query_response}
\end{table}


==> table-datasets.tex <==
\begin{table*}[b]
\resizebox{\textwidth}{!}{

\begin{tabular}{lccll}

\hline
\textbf{Dataset} & \textbf{\#Train} & \textbf{\#Test} & \textbf{Example Question} & \textbf{Description} \\ \hline



\colorg    & \colorg   & \colorg     & \colorg \texttt{Claire makes a 3 egg omelet every morning}      & multi-step  \colorg   \\
\colorg \textbf{GSM8K}~\cite{cobbe2021training}& \colorg 7473 & \colorg 1319 & \colorg  \texttt{for breakfast. How many dozens of eggs will}  & arithmetic word  \colorg    \\
\colorg & \colorg & \colorg & \colorg \texttt{she eat in 4 weeks?} & problems \colorg  \\


 &    &   &  \texttt{A trader sold an article at a profit of 20\%}      &   multi-step  \\
\textbf{AquaRat}~\cite{aqua_rat}& 97467 & 254 &  \texttt{for Rs.360. What is the cost price of the} & arithmetic word  \\
&  & & \texttt{article?} & problems  \\



\colorg   & \colorg    & \colorg   & \colorg  \texttt{Allie kept track of how many kilometers she}      & \colorg Table based   \\
\colorg \textbf{TabMWP}~\cite{tabmwp} & \colorg 23059 & \colorg 7686 & \colorg  \texttt{walked during the past 5 days. What is the} &\colorg numerical     \\
\colorg & \colorg & \colorg  & \colorg \texttt{range of the numbers?} &\colorg reasoning \\


 &    &   & \texttt{In 2010 and 2009, what was total fair value}      & Table and Text  \\
\textbf{FinQA}~\cite{chen2022finqa} & 6251 & 1147 & \texttt{in billions of assets segregated for benefit}      & based numerical  \\
& & & \texttt{of securities and futures brokerage customers?}      & reasoning
\\


\colorg   & \colorg    & \colorg   & \colorg  \texttt{Would the chef at Carmine's restaurant panic}      & \colorg multi-step   \\
\colorg \textbf{StrategyQA}~\cite{geva2021did} & \colorg 1800 & \colorg 490 & \colorg  \texttt{if there was no basil?} &\colorg reasoning     \\



\bottomrule
\end{tabular}
}
\caption{Overview of the Complex QA datasets used in this study.}
\label{tab:datasets_overview}
\end{table*}

==> table-qualitative.tex <==



\begin{table*}
\begin{tabular}{lp{.80\textwidth}}
\toprule
    \textbf{Method}     & \textbf{Decomposition} \\
\midrule


\colorg \textbf{Question}  & \colorg \textbf{In 2010 and 2009 , what was the total fair value in billions of assets segregated for the benefit of securities and futures brokerage customers?} [Dataset: \textbf{FinQA}] \\
\COT{}  & To find the total fair value in billions of assets segregated for the benefit of securities and futures brokerage customers in 2010 and 2009, we need to look at the table. \textcolor{red}{In 2010, the fair value was \$25.0 billion and in 2009, it was \$24.0 billion. Hence total is \textbf{Answer:} \$49 billion.}  \\
\colorg \icat{} + \ftd{} & \colorg \textbf{Rationale:} To find the total fair value in billions [\dots], look at the table for the years 2010 and 2009. In the table, under "year ended December 31," we can see two columns [\dots], there is a row labeled "securities and futures brokerage customers." In this row, there are values listed in millions.To convert these values to billions, we divide each value by 1000.
\textcolor{teal}{For 2010: \$25.0 billion (segregated cash) + \$9.7 billion (fair value of securities) = \$34.7 billion
For 2009: \$24.0 billion (segregated cash) + \$10.2 billion (fair value of securities) = \$34.2 billion
[\dots] \textbf{Answer:} 68.9}
 \\
\icat{} & in billions, we need to look at Note 29 in the text. 
In 2010, \$25.0 billion in cash and \$9.7 billion in securities with [\dots]. 
In 2009, \$24.0 billion in cash and \$10.2 billion in securities [\dots].
\textbf{Answer}: \texttt{68.9 (billion)}. \\
\midrule
\midrule


\end{tabular}
\caption{Qualitative analysis of reasoning chains generated by chain-of-thought vs \icat{}}
\label{tab:qualitative}
%\vspace{-0.25cm}
\end{table*}



==> table-result-exhaustive-evaluation.tex <==

\begin{table}[!t]
    \footnotesize
    \centering
     \resizebox{\linewidth}{!}{%
    \begin{tabular}{lccccc}
    \toprule
    \small

\textbf{Datasets} & \textbf{GSM} & \textbf{Aqua} & \textbf{Tab} & \textbf{Fin} & \textbf{Strat}\\


    
    \midrule

    Exhaustive eval &76.72   &50.39   &  82.24 &  57.02 & 82.45\\

    \static{} (-exploration) & 75.89& 50.00& 75.16 & 50.30 & 80.40\\
    \ \hspace{4em} (Mistral) & \\
    
    \textbf{\static{}(Llama)} & \textbf{79.07}  & \textbf{53.94}  & 80.11  &  54.66 & \textbf{85.31} \\

    \textbf{\static{}(Mistral)} & \textbf{77.86}  & \textbf{53.54}  & \textbf{83.07}  &  \textbf{59.46} & \textbf{85.71} \\
    
      \bottomrule
    \end{tabular}
    } 
    \caption{Ablation studies: exhaustive evaluation, w/o exploration vs proposed exploration (\static{}).}
    % \vspace{-1cm}
    \label{tab:exhaustive_evaluation}
\end{table}


==> table-results-SOTA.tex <==
\begin{table*}[t]
    \footnotesize
    \small

    \centering

     \resizebox{\textwidth}{!}{%
    \begin{tabular}{llllll}

    \toprule
     \textbf{Method}& \multicolumn{1}{l}{\textbf{GSM8K}}& \multicolumn{1}{l}{\textbf{AquaRat}} & \multicolumn{1}{l}{\textbf{TabMWP}} & \multicolumn{1}{l}{\textbf{FinQA}} 
     & \multicolumn{1}{l}{\textbf{StrategyQA}}  
     \\
     
    %     \midrule
    
    % SOTA & \bf \colorit 37.60  & \colorit  \bf 50.59 &   60.5  &  47.3 \\
    
    \midrule
    % \colorg \textbf{gpt-3.5-turbo} & \colorg& \colorg& \colorg& \colorg\\
       \colorg \textbf{dynamic} & \colorg & \colorg & \colorg & \colorg & \colorg \\
    KNN  \cite{rubin-etal-2022-learning}              &53.45    &51.96    &77.07   &51.52  & 81.83    \\
        KNN (S-BERT)  \cite{rubin-etal-2022-learning}              &53.07    &52.75    &77.95   &52.65  & 81.83    \\
    MMR  \cite{ye-etal-2023-complementary}            &54.36    &51.18    &77.32   &49.87    & 82.86  \\
    KNN+SC \cite{wang2022self}                        &80.21    &62.59    &83.08   &54.49 & 83.88     \\
    MMR+SC \cite{wang2022self}                        &78.01    &59.45    &81.36   &50.74  & 83.88    \\
    PromptPG \cite{lu2023dynamic}                     & \centering -       & -       &68.23   &53.56  & -    \\
    % \color{red}DQ-LoRe \color{black} \cite{xiong2023dq} & \centering -       & -       &-   &-  & -    \\


    \colorg \textbf{static} & \colorg& \colorg& \colorg& \colorg & \colorg \\
    Zero-Shot COT \cite{kojima2023large}              &67.02    &49.60    &57.10   &47.51 & 59.75         \\
    Manual Few-Shot COT \cite{wei2023chainofthought}  &73.46    &44.88    &71.22   &52.22 & 73.06     \\
    Random                                            &67.79    &49.80    &55.89   &53.70 &  81.02     \\
    PS+ \cite{wang-etal-2023-plan}                    &59.30    &46.00    & -      & -   & -      \\
    Auto-COT \cite{zhang2023automatic}                &57.10    &41.70    & -      & -  & 71.20       \\
    GraphCut \cite{iyer2013submodular}                &66.19    &47.24    &60.45   &52.31 & 80.00    \\ 
    FacilityLocation \cite{iyer2013submodular}        &68.61    &48.43    &67.66   &36.79 &  81.63    \\ 
    LENS \cite{li2023finding}                         &69.37    &48.82    &77.27  &54.75  & 79.79    \\ 
    LENS+SC \cite{li2023finding}                         &79.37    & 57.87   &  80.68 & 60.06   & 82.24  \\ 

     \colorg \textbf{Our Approach} & \colorg& \colorg& \colorg& \colorg & \colorg\\
     
    \textbf{\static{}}                 &\colorit 77.86\up{12.24} $\dagger$ &\colorit 53.54\up{9.67}$\dagger$ &\colorit 83.07\up{7.51} $\dagger$ &\colorit 59.46\up{8.60} $\dagger$ &\colorit 85.71\up{5.63} $\dagger$\\
    
    \textbf{\static{}+\selfcon{}}      &\textbf{86.35}\up{24.48} $\ddagger$&63.39\up{29.84} $\ddagger$  &85.52\up{10.68} $\ddagger$   &64.52\up{17.84}  $\ddagger$ & 87.14 \up{9.21}$\dagger$   \\
    
    \textbf{\static{}+\knn+\selfcon{}} &85.14 \up{22.73}$\ddagger$  & 62.20\up{27.41}$\ddagger$ & 86.29\up{12.39} $\ddagger$  &\textbf{65.12}\up{18.94}  $\ddagger$ & \textbf{88.37}\up{10.75}$\dagger$   \\
    
    \textbf{\static{}+\mmr+\selfcon{}} &86.13\up{24.16} $\ddagger$ &\textbf{63.78}\up{30.64} $\ddagger$&\textbf{86.96}\up{12.54}$\ddagger$    &64.60\up{17.99}   $\ddagger$    & 87.55\up{9.73}$\dagger$       \\


  
    
%     \midrule
%     \colorg \textbf{Mistral} & \colorg& \colorg& \colorg& \colorg\\
% %     \colorg \textbf{dynamic} & \colorg& \colorg& \colorg& \colorg\\
% % KNN                         &37.98  &23.22 &61.74 &9.06   \\ 
% %     KNN+SC                      &61.71  &35.02 &67.98 &11.33  \\
% %     MMR                         &46.25  &18.11 &52.82 &10.11  \\
% %     MMR+SC                      &62.24  &33.07 &65.08 &12.03  \\
% %         \colorg \textbf{static} & \colorg& \colorg& \colorg& \colorg\\
%     Zero-Shot COT               &7.43   &      &43.34 &       \\
%     Few Shot COT                &30.48  &14.90 &46.94 &       \\
%     Random                      &33.81  &22.04 &30.40 &5.52   \\ 
%     LENS                        &       &      &      &       \\ 
    
%     \static{}                   &45.41  &30.07 &48.79 &5.57   \\
%     \static{}+\selfcon{}        &61.41  &34.10 &61.96 &7.41   \\
%     \static{}+\knn+\selfcon{}   &62.92  &23.22 &59.91 &4.79   \\
%     \static{}+\mmr+\selfcon{}   &60.05  &22.44 &61.29 &5.40   \\
%     \static{}+\pot{}+\selfcon{} &56.33  &26.00 &61.24 &10.11  \\

%     \midrule
%     \colorg \textbf{Llama-2-7B} & \colorg& \colorg& \colorg& \colorg\\

%     %     \colorg \textbf{dynamic} & \colorg& \colorg& \colorg& \colorg\\
%     % KNN                         &23.43  &28.34 &54.83 &10.37  \\
%     % KNN+SC                      &39.80  &34.8  &64.18 &11.33  \\
%     % MMR                         &29.64  &21.65 &49.61 &12.20  \\
%     % MMR+SC                      &38.74  &27.16 &56.99 &12.90  \\
%     %       \colorg \textbf{static} & \colorg& \colorg& \colorg& \colorg\\ 
%     Zero-Shot COT               &6.14   &      &40.31 &       \\
%     Few Shot COT                &21.15  &20.47 &43.23 &       \\
%     Random                      &18.27  &21.6  &28.41 &4.62   \\ 
%     LENS                        &       &      &      &       \\ 

%     \static{}                   &27.67  &24.40 &46.25 &6.62   \\
%     \static{}+\selfcon{}        &36.85  &24.01 &56.74 &6.21   \\
%     \static{}+\knn+\selfcon{}   &38.21  &22.83 &49.80 &5.92   \\
%     \static{}+\mmr+\selfcon{}   &38.60  &26.77 &51.68 &6.36   \\
%     \static{}+\pot{}+\selfcon{} &23.35  &      &45.44 &10.28  \\
%  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    % random &  20.28& 25.33&  81.71 & 74.7  \\
    
    % \mmr+\selfcon{} &  1.59 & 20.00 &  10.25 & 8.31  \\
      
    % \static{}+\selfcon{} &  25.24$\dagger$&  34.00& \colorit  96.14 $\dagger$ & \coloritt  80.0  \\
      
    % \static{}+\pot{}+\selfcon{} &  24.92$\dagger$&  34.00& \colorit   $\dagger$ & \coloritt     \\


%         \midrule
%  \colorg \textbf{Mistral} & \colorg& \colorg& \colorg& \colorg\\
  
%     random &  20.28& 25.33&  81.71 & 74.7  \\
    
%     \mmr{}+\selfcon{} &  1.59 & 20.00 &  10.25 & 8.31  \\
      
%     \static{}+\selfcon{} &  25.24$\dagger$&  34.00& \colorit  96.14 $\dagger$ & \coloritt  80.0  \\
      
%     \static{}+\pot{}+\selfcon{} &  24.92$\dagger$&  34.00& \colorit   $\dagger$ & \coloritt     \\


%       \midrule
% \colorg \textbf{Llama-2-7B} &\colorg & \colorg& \colorg& \colorg\\

%    random&  24.36& 29.41&  92.95 &   77.60  \\

%     \mmr+\selfcon{}  &  26.99& 30.69&  \coloritt  95.13 & \colorit  80.70  \\
    
%      \static{}+\selfcon{}  &  27.07& 30.33&  94.96 & \colorit  80.70  \\
     
%     \static{}+\pot{}+\selfcon{} &  \coloritt  \textbf{27.24}$\ddagger$& \coloritt  \textbf{36.00}&  \colorit  \textbf{96.14}$\dagger$ & \colorit  \textbf{80.70}  \\



 %        \midrule
 % \colorg \textbf{FLAN-T5-XL} & \colorg& \colorg& \colorg& \colorg\\
  
 %    random &  20.28& 25.33&  81.71 & 74.7  \\
    
 %    \mmr{}+\selfcon{} &  1.59 & 20.00 &  10.25 & 8.31  \\
      
 %    \static{}+\selfcon{} &  25.24$\dagger$&  34.00& \colorit  96.14 $\dagger$ & \coloritt  80.0  \\
      
 %    \static{}+\pot{}+\selfcon{} &  24.92$\dagger$&  34.00& \colorit   $\dagger$ & \coloritt     \\
     
     \bottomrule
    \end{tabular}
    } 
    \caption{Results across datasets using gpt-3.5-turbo model as backbone. Percentage improvements are reported over LENS \cite{li2023finding}.  $\dagger$ indicates statistical significance using t-test over LENS at 0.05 level and $\ddagger$  at 0.01 level.}
    % \vspace{-1cm}
    \label{tab:main_result}
\end{table*}

% \color{purple} SB: Can we split this table into two - first one with only GPT3 results claiming state of the art performance (add a lot more baseline results), and second one improvement over other exemplar selection techniques ?






==> table-results-llm-calls.tex <==
\begin{table*}[t]
    \centering
    % resizebox{\textwidth}{!}{% 
    \begin{tabular}{lccccccc}
    \toprule

\textbf{Datasets} & \textbf{\begin{tabular}[c]{@{}c@{}}Zero-Shot \\ COT\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Few-Shot\\  COT\end{tabular}} & \textbf{Random} & \textbf{KNN}  & \textbf{MMR}  & \textbf{LENS} & \textbf{Explora} \\
    
     % \textbf{Datasets}& \multicolumn{1}{c}{\textbf{Zero-Shot COT}}& \multicolumn{1}{c}{\textbf{Few-shot COT}} & \multicolumn{1}{c}{\textbf{Random}} & \multicolumn{1}{c}{\textbf{KNN}} & \multicolumn{1}{c}{\textbf{MMR}} & \multicolumn{1}{c}{\textbf{LENS}} & \multicolumn{1}{c}{\textbf{Explora}}  \\
    

    \midrule

    \textbf{GSM8K}    &1319   &1319   &1319   &1319    &1319    &24176     &4719   \\
    \textbf{AquaRat}  &254    &254    &254    &254     &254     &23111     &3654   \\
    \textbf{TabMWP}   &7686   &7686   &7686   &7686    &7686    &30543     &11086  \\
    \textbf{FinQA}    &1147   &1147   &1147   &1147    &1147    &24004     &4547   \\
      \bottomrule
    \end{tabular}
    % } 
    \caption{Frugal subset selection approach - we reduce number of calls to LLMs. Our score based approach enables us to make fewer calls to LLMs compared to LENS which lacks this score based modelling.}
    % \vspace{-1cm}
    \label{tab:llm_calls}
\end{table*}


==> table-results-llms_transfer.tex <==
\begin{table}[!t]
\footnotesize
    \centering
    \small
     \resizebox{\linewidth}{!}{%
    \begin{tabular}{lcccccc}
    \toprule
    
     \textbf{Method}& \multicolumn{1}{c}{\textbf{T}} & \multicolumn{1}{c}{\textbf{GSM}}& \multicolumn{1}{c}{\textbf{Aqua}} & \multicolumn{1}{c}{\textbf{Tab}} & \multicolumn{1}{c}{\textbf{Fin}}
     & \multicolumn{1}{c}{\textbf{Strat}} \\
     

    %     \midrule
    
    % SOTA & \bf \colorit 37.60  & \colorit  \bf 50.59 &   60.5  &  47.3 \\
    
    \midrule
    % \colorg \textbf{gpt-3.5-turbo} & \colorg& \colorg& \colorg& \colorg\\

    \textbf{\staticshort{}}                &  L    &79.07  &53.94  & 80.11     &  54.66  & 85.31    \\
                             &  M   &77.86  &53.54  & 83.07     &  59.46 & 85.71    \\
    \textbf{\staticshort{}+\selfcon{}}     &  L    &85.82  &63.78  & 86.76     &  61.16  & 85.10   \\
                             &  M   &86.35  &63.39  & 85.52     &  64.52  & 87.14    \\
    \textbf{\staticshort{}+\knn+\selfcon{}}&  L    &85.89  &64.17  & 85.74     &  63.64  & 86.53   \\
                             &  M   &85.14  &62.20  & 86.29     &  65.12 & 88.37    \\
    \textbf{\staticshort{}+\mmr+\selfcon{}}&  L    &86.20  &62.99  & 87.81     &  64.60  & 86.12   \\
                             &  M   &86.13  &63.78  & 86.96     &  64.60   & 87.55  \\



     \bottomrule
    \end{tabular}
    } 
    \caption{Results for transfer (T) of exemplars selected using \static{} (\staticshort{}) on smaller LLMs (Llama2-7b (L) and Mistral-7b (M)) to larger LLM (gpt-3.5-turbo).}
    % \vspace{-1cm}
    \label{tab:llm_transfer}
\end{table}








==> table-results-robustness.tex <==
% \begin{table*}[t]
%     \footnotesize
%     \centering
%     % resizebox{\textwidth}{!}{% 
%     \begin{tabular}{lccccccccc}
%     \toprule

% \textbf{Datasets} & \textbf{\begin{tabular}[c]{@{}c@{}}Zero-Shot \\ COT\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Few-Shot\\  COT\end{tabular}}  & \textbf{KNN}  & \textbf{MMR}  & \textbf{\begin{tabular}[c]{@{}c@{}}Graph \\ Cut\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}Facility \\ Location\end{tabular}}  & \textbf{LENS} & \textbf{Explora} \\
    
%      % \textbf{Datasets}& \multicolumn{1}{c}{\textbf{Zero-Shot COT}}& \multicolumn{1}{c}{\textbf{Few-shot COT}} & \multicolumn{1}{c}{\textbf{Random}} & \multicolumn{1}{c}{\textbf{KNN}} & \multicolumn{1}{c}{\textbf{MMR}} & \multicolumn{1}{c}{\textbf{LENS}} & \multicolumn{1}{c}{\textbf{Explora}}  \\
    

%     \midrule

%     \textbf{GSM8K}    & $\pm$5.18   & $\pm$4.48     &  $\pm$3.76 & $\pm$4.00   & $\pm$6.38  &  $\pm$4.23&  $\pm$5.04     & \textbf{$\pm$3.39}  \\
%     \textbf{AquaRat}  & $\pm$7.08  &  $\pm$12.03 & $\pm$5.49  &  $\pm$10.53  &  $\pm$8.18  & $\pm$6.71  & $\pm$6.67 & \textbf{$\pm$4.93}  \\
%     \textbf{TabMWP}   & $\pm$1.84   & $\pm$1.66  &  $\pm$1.27 &  $\pm$1.68  & $\pm$2.03   &  $\pm$1.74    & $\pm$1.72 & $\pm$1.45 \\
%     \textbf{FinQA}    & $\pm$4.50  & $\pm$4.76  & $\pm$4.17  &  $\pm$6.10  & $\pm$5.29   &  $\pm$4.94 &  $\pm$5.81 & \textbf{$\pm$3.41}  \\
%       \bottomrule
%     \end{tabular}
%     % } 
%     \caption{Comparison of robustness of \static{} to other approaches. We report standard deviation (lower is better) using scores from different splits of test set.}
%     % \vspace{-1cm}
%     \label{tab:robustness}
% \end{table*}













\begin{table}[!t]
    \footnotesize
    \centering
     \resizebox{\linewidth}{!}{%
    \begin{tabular}{lccccc}
    \toprule
    \small

\textbf{Datasets} & \textbf{GSM} & \textbf{Aqua} & \textbf{Tab} & \textbf{Fin} & \textbf{Strat}\\

% \textbf{\begin{tabular}[c]{@{}c@{}}Zero-Shot \\ COT\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Few-Shot\\  COT\end{tabular}}  & \textbf{KNN}  & \textbf{MMR}  & \textbf{\begin{tabular}[c]{@{}c@{}}Graph \\ Cut\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}Facility \\ Location\end{tabular}}  & \textbf{LENS} & \textbf{Explora} \\
    
    \midrule

    Zero-Shot COT    & $\pm$5.18   & $\pm$7.08     &  $\pm$1.84 & $\pm$4.50 & $\pm$4.19     \\
    Few-Shot COT  & $\pm$4.48  &  $\pm$12.03 & $\pm$1.66  &  $\pm$4.76 & $\pm$5.67   \\
    KNN   & $\pm$3.76   & $\pm$5.49  &  $\pm$1.27 &  $\pm$4.17  & $\pm$4.85 \\
    MMR    & $\pm$4.00  & $\pm$10.53  & $\pm$1.68  &  $\pm$6.10 &  $\pm$5.70  \\
    Graph Cut & $\pm$6.38& $\pm$8.18  & $\pm$2.03  &  $\pm$5.29 & $\pm$7.62 \\
    Facility Location & $\pm$4.23  & $\pm$6.71  & $\pm$1.74  &  $\pm$4.94 & $\pm$5.93 \\
    LENS & $\pm$5.04  & $\pm$6.67  & $\pm$1.59  &  $\pm$5.81 & $\pm$ 3.98 \\
    \textbf{\static{}} & $\pm$\textbf{3.39}  & $\pm$\textbf{4.93}  & $\pm$1.50  &  $\pm$\textbf{3.41} &$\pm$ \textbf{3.95} \\
    
      \bottomrule
    \end{tabular}
    } 
    \caption{Comparison of robustness of \static{} to other approaches. We report standard deviation (lower is better) with scores from different splits of eval. set.}
    % \vspace{-1cm}
    \label{tab:robustness}
\end{table}


==> table-results-small-models.tex <==
\begin{table*}[hbt!]
    \centering
    % resizebox{\textwidth}{!}{% 
    \begin{tabular}{lcccc}
    \toprule
    
     \textbf{Method}& \multicolumn{1}{c}{\textbf{GSM8K}}& \multicolumn{1}{c}{\textbf{AquaRat}} & \multicolumn{1}{c}{\textbf{TabMWP}} & \multicolumn{1}{c}{\textbf{FinQA}} \\
     

    %     \midrule
    
    % SOTA & \bf \colorit 37.60  & \colorit  \bf 50.59 &   60.5  &  47.3 \\
    
    \midrule
    \colorg \textbf{Mistral-7B} & \colorg& \colorg& \colorg & \colorg \\\\
       \colorg \textbf{dynamic} & \colorg & \colorg & \colorg & \colorg   \\
    KNN  \cite{rubin-etal-2022-learning}             &37.98  &23.22    &61.74   & 9.06       \\
    MMR  \cite{ye-etal-2023-complementary}           &46.25  &18.11    &52.82   & 10.11      \\
    % KNN+SC \cite{wang2022self}                       &61.71  &35.02    &67.98   & 11.33      \\
    % MMR+SC \cite{wang2022self}                       &62.24  &33.07    &65.08   & 12.03      \\
    % PromptPG \cite{lu2023dynamic}                  & -     & -       & 68.23  & 53.56      \\


    \colorg \textbf{static} & \colorg& \colorg& \colorg& \colorg\\
    Zero-Shot COT \cite{kojima2023large}             &7.43   &21.65    &43.34   &1.74        \\
    Manual Few-shot COT \cite{wei2023chainofthought} &30.48  &14.90    &46.94   &3.22        \\
    Random                                           &33.81  &22.04    &30.40   &5.52        \\
    % PS+ \cite{wang-etal-2023-plan}                 &59.30  &46.00    & -      & -          \\
    % Auto-COT \cite{zhang2023automatic}             &57.10  &41.70    & -      & -          \\
    GraphCut \cite{iyer2013submodular}               &47.00  &21.65    &59.46   &5.66        \\ 
    FacilityLocation \cite{iyer2013submodular}       &46.25  &14.17    &57.74   &4.96        \\ 
    LENS \cite{li2023finding}                        &46.39  &29.92    &57.69   &5.14        \\ 


    \colorg \textbf{Our Approach} & \colorg& \colorg& \colorg& \colorg \\
    \static{}                                        & 46.41  &30.07    &58.62   &5.57        \\
    \static{}+\selfcon{}                     &\textbf{61.41}  &\textbf{35.10}   &\textbf{61.96}   &7.41        \\
    % \static{}+\knn+\selfcon{}               &\textbf{62.92}  &23.22    &59.91   &4.79        \\
    % \static{}+\mmr+\selfcon{}                        &60.05  &22.44    &61.29   &5.40        \\
    % \static{}+\pot{}+\selfcon{} &76.87  &      &      &   \\



\midrule
    \colorg \textbf{Llama2-7B} & \colorg& \colorg& \colorg& \colorg \\\\
       \colorg \textbf{dynamic} & \colorg & \colorg & \colorg & \colorg  \\
    KNN  \cite{rubin-etal-2022-learning}             &23.43  &28.34    &54.83   & 10.37      \\
    MMR  \cite{ye-etal-2023-complementary}           &29.64  &21.65    &49.61   & 12.20      \\
    % KNN+SC \cite{wang2022self}                       &38.80  &34.80    &64.18   & 11.33      \\
    % MMR+SC \cite{wang2022self}                       &38.74  &27.16    &56.99   & 12.90      \\
    % PromptPG \cite{lu2023dynamic}                  & -     & -       & 68.23  & 53.56      \\


    \colorg \textbf{static} & \colorg& \colorg& \colorg& \colorg \\
    Zero-Shot COT \cite{kojima2023large}             &6.14   &6.29     &40.31   &1.67        \\
    Manual Few-shot COT \cite{wei2023chainofthought} &21.15  &20.47    &43.23   &2.87        \\
    Random                                           &18.27  &21.60    &28.41   &4.62        \\
    % PS+ \cite{wang-etal-2023-plan}                 &59.30  &46.00    & -      & -          \\
    % Auto-COT \cite{zhang2023automatic}             &57.10  &41.70    & -      & -          \\
    GraphCut \cite{iyer2013submodular}               &27.29  &21.65    &47.38   &5.40        \\ 
    FacilityLocation \cite{iyer2013submodular}       &27.21  &21.65    &47.23   &5.05        \\ 
    LENS \cite{li2023finding}                        &28.05  &23.22    &48.29   &6.62        \\ 


    \colorg \textbf{Our Approach} & \colorg& \colorg& \colorg& \colorg \\
    \static{}                                        &28.67  &24.40    &49.96   &6.62        \\
    \static{}+\selfcon{}                             &\textbf{36.85}  &24.01    & \textbf{56.74}  &6.21        \\
    % \static{}+\knn+\selfcon{}                        &38.21  &22.83    &49.80   &5.92        \\
    % \static{}+\mmr+\selfcon{}               &\textbf{38.90}  &26.77    &51.68   &6.36        \\
    % \static{}+\pot{}+\selfcon{} &76.87  &      &      &   \\

  
    
     \bottomrule
    \end{tabular}
    % } 
    \caption{Results across datasets on \mistral{} and \llamaseven{}.}
    % \vspace{-1cm}
    \label{tab:main_result_small_models}
\end{table*}








==> table-results-v2.tex <==
\begin{table*}[!t]
    \centering
    
    \begin{tabular}{lcccc}
    \toprule
    
     \textbf{Method}& \multicolumn{1}{c}{\aqua{}}& \multicolumn{1}{c}{\strat{}} & \multicolumn{1}{c}{\advhotpot{}} & \multicolumn{1}{c}{\tab{}}  \\
     
     % & cover-EM & cover-EM& EM& EM&EM \\
    %  \midrule
    %  \fshot{}& 11.66& 28.41& 85.74& 78.2& 42.55\\
     
    %  \COT{} &20.85& 34.08&94.79&  79.4&52.22 \\
     
    %  \zfshot{} & 12.22& 19.25& 88.75& 75.4& 47.51 \\
    % \hline
    % \self{} & 23.64& 32.58& N/A& N/A& N/A \\
      
    %   \autocot{} &  N/A& N/A&  93.83 & 76.2 & N/A \\

        \midrule
    
    SOTA & \bf \colorit 37.60  & \colorit  \bf 50.59 &   60.5  &  47.3 \\
    
        \midrule
 \colorg \textbf{gpt-3.5-turbo} & \colorg& \colorg& \colorg& \colorg\\
  
    random &  20.28& 25.33&  81.71 & 74.7  \\
    
    \mmr+\selfcon{} &  1.59 & 20.00 &  10.25 & 8.31  \\
      
    \static{}+\selfcon{} &  25.24$\dagger$&  34.00& \colorit  96.14 $\dagger$ & \coloritt  80.0  \\
      
    \static{}+\pot{}+\selfcon{} &  24.92$\dagger$&  34.00& \colorit   $\dagger$ & \coloritt     \\


        \midrule
 \colorg \textbf{Mistral} & \colorg& \colorg& \colorg& \colorg\\
  
    random &  20.28& 25.33&  81.71 & 74.7  \\
    
    \mmr{}+\selfcon{} &  1.59 & 20.00 &  10.25 & 8.31  \\
      
    \static{}+\selfcon{} &  25.24$\dagger$&  34.00& \colorit  96.14 $\dagger$ & \coloritt  80.0  \\
      
    \static{}+\pot{}+\selfcon{} &  24.92$\dagger$&  34.00& \colorit   $\dagger$ & \coloritt     \\


      \midrule
\colorg \textbf{Llama-2-7B} &\colorg & \colorg& \colorg& \colorg\\

   random&  24.36& 29.41&  92.95 &   77.60  \\

    \mmr+\selfcon{}  &  26.99& 30.69&  \coloritt  95.13 & \colorit  80.70  \\
    
     \static{}+\selfcon{}  &  27.07& 30.33&  94.96 & \colorit  80.70  \\
     
    \static{}+\pot{}+\selfcon{} &  \coloritt  \textbf{27.24}$\ddagger$& \coloritt  \textbf{36.00}&  \colorit  \textbf{96.14}$\dagger$ & \colorit  \textbf{80.70}  \\



        \midrule
 \colorg \textbf{FLAN-T5-XL} & \colorg& \colorg& \colorg& \colorg\\
  
    random &  20.28& 25.33&  81.71 & 74.7  \\
    
    \mmr{}+\selfcon{} &  1.59 & 20.00 &  10.25 & 8.31  \\
      
    \static{}+\selfcon{} &  25.24$\dagger$&  34.00& \colorit  96.14 $\dagger$ & \coloritt  80.0  \\
      
    \static{}+\pot{}+\selfcon{} &  24.92$\dagger$&  34.00& \colorit   $\dagger$ & \coloritt     \\
     
     \bottomrule
    \end{tabular}
    \caption{Results across datasets. $\dagger$ and $\ddagger$ indicates statistical significance over \COT{} at 0.1 level  and 0.01 level respectively. SOTA results are included for completion.}
    % \vspace{-1cm}
    \label{tab:main_result}
\end{table*}


==> table_category_perf.tex <==
\begin{table*}[ht]
\centering

\renewcommand{\arraystretch}{1.3} % Increase row height
\begin{tabular}{llcccccc}
\toprule
\textbf{Model} & \textbf{Type} & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c}{\textbf{Recall}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{Temporal Overlap}} & \multicolumn{1}{c}{\textbf{Time Jaccard}} \\
\midrule
\multicolumn{7}{>{\columncolor[gray]{0.93}}l}{\textbf{Closed Book}} \\
\multirow{2}{*}{Mistral KNN} & Sports & 0.469 & 0.245 & 0.308 & 0.420 & 0.322 \\
 & Political & 0.593 & 0.374 & 0.423 & 0.459 & 0.402 \\
\multirow{2}{*}{Meta Llama KNN} & Sports & 0.512 & 0.357 & 0.408 & 0.467 & 0.358 \\
 & Political & 0.583 & 0.440 & 0.477 & 0.568 & 0.493 \\

\multicolumn{7}{>{\columncolor[gray]{0.93}}l}{\textbf{Open Book}} \\
\multirow{2}{*}{Mistral BM25} & Sports & 0.800 & 0.545 & 0.630 & 0.730 & 0.675 \\
 & Political & 0.690 & 0.606 & 0.619 & 0.571 & 0.535 \\
\multirow{2}{*}{Mistral all-mini-lm} & Sports & 0.516 & 0.294 & 0.358 & 0.419 & 0.350 \\
 & Political & 0.628 & 0.463 & 0.503 & 0.424 & 0.393 \\
\multirow{2}{*}{Mistral Multi QA} & Sports & 0.517 & 0.312 & 0.373 & 0.433 & 0.348 \\
 & Political & 0.634 & 0.474 & 0.511 & 0.445 & 0.411 \\

\multicolumn{7}{>{\columncolor[gray]{0.93}}l}{\textbf{Golden Evidence}} \\
\multirow{2}{*}{Mistral Golden Manual} & Sports & 0.941 & 0.661 & 0.763 & 0.862 & 0.818 \\
 & Political & 0.898 & 0.876 & 0.874 & 0.634 & 0.613 \\
\multirow{2}{*}{Mistral Golden KNN} & Sports & 0.935 & 0.760 & 0.828 & 0.897 & 0.847 \\
 & Political & 0.949 & 0.940 & 0.935 & 0.816 & 0.792 \\
\bottomrule
\end{tabular}
\caption{Performance of various models on the benchmark using different prompting techniques, categorized by question type (Sports and Political) using Mistral v0.2}
\label{tab:sports_vs_political_performance}
\end{table*}
